Learning Robust Real-Time Cultural Transmission without Human Data

Cultural transmission is the domain-general social skill that allows agents to acquire and use information from each other in real-time with high fidelity and recall. In humans, it is the inheritance process that powers cumulative cultural evolution, expanding our skills, tools and knowledge across generations. We provide a method for generating zero-shot, high recall cultural transmission in artificially intelligent agents. Our agents succeed at real-time cultural transmission from humans in novel contexts without using any pre-collected human data. We identify a surprisingly simple set of ingredients sufficient for generating cultural transmission and develop an evaluation methodology for rigorously assessing it. This paves the way for cultural evolution as an algorithm for developing artificial general intelligence.

==> Cultural General Intelligence (Final Copy for arXiv)/authors_and_contributions.tex <==

\section{Authors and contributions}
\label{authors}

Below is a list of authors and contributors listed alphabetically by last name. Each name is followed by the contributions of the individual.

\begin{itemize}
    \item \textbf{Avishkar Bhoopchand}: Learning process development, research investigations, infrastructure development, technical management, manuscript editing.
    \item \textbf{Bethanie Brownfield}: Quality assurance testing.
    \item \textbf{Adrian Collister}: Environment development.
    \item \textbf{Agustin Dal Lago}: Agent analysis, infrastructure development, code quality.
    \item \textbf{Ashley Edwards}: Research investigations, agent analysis. 
    \item \textbf{Richard Everett}: Cultural general intelligence concept, agent analysis, learning process development, research investigations, infrastructure development, additional environment design, technical management, team management.
    \item \textbf{Alexandre Fr\'echette}: Infrastructure development.
    \item \textbf{Yanko Gitahy Oliveira}: Environment development.
    \item \textbf{Edward Hughes}: Cultural general intelligence concept, research investigations, infrastructure development, team management, manuscript editing. 
    \item \textbf{Kory W. Mathewson}: Learning process development, research investigations, agent analysis, team management.
    \item \textbf{Piermaria Mendolicchio}: Quality assurance testing.
    \item \textbf{Julia Pawar}: Program management.
    \item \textbf{Miruna P\^{i}slar}: Learning process development, research investigations, agent analysis, infrastructure development.
    \item \textbf{Alex Platonov}: Environment visuals.
    \item \textbf{Evan Senter}: Infrastructure development, technical management, team management.
    \item \textbf{Sukhdeep Singh}: Program management. 
    \item \textbf{Alexander Zacherl}: Environment design, environment development, agent analysis.
    \item \textbf{Lei M.~Zhang}: Learning process development, research investigations, infrastructure development, technical management.
    
\end{itemize}

\paragraph{Corresponding authors:} Edward Hughes (\href{mailto:edwardhughes@deepmind.com}{\nolinkurl{edwardhughes@deepmind.com}}), Richard Everett (\href{mailto:reverett@deepmind.com}{\nolinkurl{reverett@deepmind.com}}).


==> Cultural General Intelligence (Final Copy for arXiv)/background.tex <==
\clearpage
\section{Learning algorithm}\label{background}

Our hypothesis is that robust cultural transmission is a ``cognitive gadget'' \citep{heyes2018cognitive}. We show that cultural transmission can be reinforcement learned purely from individual reward \citep{SILVER2021103535}. We require only that the environment contains knowledgeable co-players and that the agent has a minimal sufficient number of representational and experiential biases (see Section \ref{sec:training}). From the perspective of an agent capable of cultural transmission from an expert, the policy of the expert must be inferred online using only the transition dynamics of the environment. In other words, the agent must solve the correspondence problem.  

If our agent learns a cultural transmission policy, it is by observing an expert agent in the world and correlating improved expected return with the ability to reproduce the other agent's behaviour. If that cultural transmission policy is robust, then reinforcement learning (RL) must have favoured imitation with high fidelity, generalising across a range of contexts, and recalling transmitted behaviours. As a basis for our claims, we use a state-of-the-art continuous control deep reinforcement learning algorithm, maximum a posteriori policy optimisation (MPO) \citep{abdolmaleki2018maximum}. For details of the RL formalism and MPO algorithm, see Appendix \ref{app:learning_algorithm}. 

A crucial challenge in RL is the balance between exploration and exploitation. Exploration involves discovering new parts of the state-action space and their implications for value; exploitation involves using learned information about valuable states and actions to gain reward \citep{kearns2002near}. Exploration is challenging when reward is sparse or deceptive and the state-action space is large. There may be many steps required to discover an improved strategy which forego the reward offered by exploitation. In such ``hard exploration'' problems, RL is prone to falling into local optima. We show how an independent agent can learn to model its environment, and particularly others therein, to solve held-out hard exploration problems.

Reinforcement learning of cultural transmission cannot occur in fully-observed tabular settings where the environment reward is unaffected by the behaviour of the expert. The proof of this is straightforward. For an agent to learn cultural transmission, they must be rewarded in states where the behaviour of an expert co-player is salient. However, in a fully observed setting, these states also contain perfect information about the environmental features. By assumption these features determine the agent's reward independently of the behaviour of the expert. If the setting is tabular, there is no aliasing of states, so the behaviour of the expert is irrelevant from the perspective of the Q-function. 

In our setting we violate the assumptions of this lemma in two ways: by operating in a partially observable setting, and by operating in a rich 3D physical world that necessitates function approximation. Under these conditions, with appropriate domain randomisation and attention biases, we show that reinforcement learning on environment reward alone is sufficient to learn a cultural transmission policy. The corresponding neural network aliases states in such a way that it can both infer hidden information from the expert and reuse that information after the expert has dropped out. 

==> Cultural General Intelligence (Final Copy for arXiv)/defns.tex <==
%
% A useful set of commands
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{booktabs}
\usepackage{xfrac}
\usepackage{bbm}

\usepackage{algorithm}
\usepackage{algorithmicx}

\usepackage[most]{tcolorbox}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{changepage}
\usepackage{enumitem}

\newcommand{\qedwhite}{\hfill \ensuremath{\Box}}

%http://www-db.stanford.edu/~manku/latex.html
%The itemize environment can be replaced by:
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }

%Example usage: \squishlist    %% \begin{itemize}
%\item First item
%\item Second item
%\squishend     %% \end{itemize}

\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}


\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}



\newcommand{\tm}{\tilde{m}}
\newcommand{\tv}{\tilde{v}}

% For bold vector symbols
\newcommand{\myvec}[1]{\boldsymbol{#1}}
\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\ind}[1]{\mathbb{I}(#1)}

\newcommand{\vzero}{\myvecsym{0}}
\newcommand{\vone}{\myvecsym{1}}
\newcommand{\valpha}{\myvecsym{\alpha}}
\newcommand{\vbeta}{\myvecsym{\beta}}
\newcommand{\vchi}{\myvecsym{\chi}}
\newcommand{\vdelta}{\myvecsym{\delta}}
\newcommand{\vDelta}{\myvecsym{\Delta}}
\newcommand{\vepsilon}{\myvecsym{\epsilon}}
\newcommand{\vell}{\myvecsym{\ell}}
\newcommand{\veta}{\myvecsym{\eta}}
\newcommand{\vgamma}{\myvecsym{\gamma}}
\newcommand{\vGamma}{\myvecsym{\Gamma}}
\newcommand{\vmu}{\myvecsym{\mu}}
\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vkappa}{\myvecsym{\kappa}}
\newcommand{\vlambda}{\myvecsym{\lambda}}
\newcommand{\vLambda}{\myvecsym{\Lambda}}
\newcommand{\vLambdaBar}{\overline{\vLambda}}
\newcommand{\vomega}{\myvecsym{\omega}}
\newcommand{\vOmega}{\myvecsym{\Omega}}
\newcommand{\vphi}{\myvecsym{\phi}}
\newcommand{\vPhi}{\myvecsym{\Phi}}
\newcommand{\vpi}{\myvecsym{\pi}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\myvecsym{\Psi}}
\newcommand{\vtheta}{\myvecsym{\theta}}
\newcommand{\vTheta}{\myvecsym{\Theta}}
\newcommand{\vsigma}{\myvecsym{\sigma}}
\newcommand{\vSigma}{\myvecsym{\Sigma}}
\newcommand{\vtau}{\myvecsym{\tau}}
\newcommand{\vupsilon}{\myvecsym{\upsilon}}
\newcommand{\vxi}{\myvecsym{\xi}}

\newcommand{\vxn}{\vx^{(n)}}

\newcommand{\vmuY}{\vb}
\newcommand{\vmuMu}{\vmu_{x}}
\newcommand{\vmuMuGivenY}{\vmu_{x|y}}
\newcommand{\vSigmaMu}{\vSigma_{x}}
\newcommand{\vSigmaMuInv}{\vSigma_{x}^{-1}}
\newcommand{\vSigmaMuGivenY}{\vSigma_{x|y}}
\newcommand{\vSigmaMuGivenYinv}{\vSigma_{x|y}^{-1}}
\newcommand{\vSigmaY}{\vSigma_{y}}
\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

%\newcommand{\vmuY}{\vmu_{y}}
%\newcommand{\vmuMu}{\vmu_{\mu}}
%\newcommand{\vmuMuGivenY}{\vmu_{\mu|y}}
%\newcommand{\vSigmaMu}{\vSigma_{\mu}}
%\newcommand{\vSigmaMuInv}{\vSigma_{\mu}^{-1}}
%\newcommand{\vSigmaMuGivenY}{\vSigma_{\mu|y}}
%\newcommand{\vSigmaMuGivenYinv}{\vSigma_{\mu|y}^{-1}}
%\newcommand{\vSigmaY}{\vSigma_{y}}
%\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

\newcommand{\muY}{\mu_{y}}
\newcommand{\muMu}{\mu_{\mu}}
\newcommand{\muMuGivenY}{\mu_{\mu|y}}
\newcommand{\SigmaMu}{\Sigma_{\mu}}
\newcommand{\SigmaMuInv}{\Sigma_{\mu}^{-1}}
\newcommand{\SigmaMuGivenY}{\Sigma_{\mu|y}}
\newcommand{\SigmaMuGivenYinv}{\Sigma_{\mu|y}^{-1}}
\newcommand{\SigmaY}{\Sigma_{y}}
\newcommand{\SigmaYinv}{\Sigma_{y}^{-1}}

\newcommand{\hatf}{\hat{f}}
\newcommand{\haty}{\hat{y}}
\newcommand{\const}{\mbox{const}}
\newcommand{\sigmoid}{\mbox{sigm}}

\newcommand{\one}{(1)}
\newcommand{\two}{(2)}

\newcommand{\va}{\myvec{a}}
\newcommand{\vb}{\myvec{b}}
\newcommand{\vc}{\myvec{c}}
\newcommand{\vd}{\myvec{d}}
\newcommand{\ve}{\myvec{e}}
\newcommand{\vf}{\myvec{f}}
\newcommand{\vg}{\myvec{g}}
\newcommand{\vh}{\myvec{h}}
\newcommand{\vj}{\myvec{j}}
\newcommand{\vk}{\myvec{k}}
\newcommand{\vl}{\myvec{l}}
\newcommand{\vm}{\myvec{m}}
\newcommand{\vn}{\myvec{n}}
\newcommand{\vo}{\myvec{o}}
\newcommand{\vp}{\myvec{p}}
\newcommand{\vq}{\myvec{q}}
\newcommand{\vr}{\myvec{r}}
\newcommand{\vs}{\myvec{s}}
\newcommand{\vt}{\myvec{t}}
\newcommand{\vu}{\myvec{u}}
\newcommand{\vv}{\myvec{v}}
\newcommand{\vw}{\myvec{w}}
\newcommand{\vws}{\vw_s}
\newcommand{\vwh}{\hat{\vw}}
\newcommand{\vx}{\myvec{x}}
%\newcommand{\vx}{\myvec{x}}
\newcommand{\vxt}{\myvec{\tilde{x}}}
\newcommand{\vy}{\myvec{y}}
\newcommand{\vyt}{\myvec{\tilde{y}}}
\newcommand{\vz}{\myvec{z}}

\newcommand{\vA}{\myvec{A}}
\newcommand{\vB}{\myvec{B}}
\newcommand{\vC}{\myvec{C}}
\newcommand{\vD}{\myvec{D}}
\newcommand{\vE}{\myvec{E}}
\newcommand{\vF}{\myvec{F}}
\newcommand{\vG}{\myvec{G}}
\newcommand{\vH}{\myvec{H}}
\newcommand{\vI}{\myvec{I}}
\newcommand{\vJ}{\myvec{J}}
\newcommand{\vK}{\myvec{K}}
\newcommand{\vL}{\myvec{L}}
\newcommand{\vM}{\myvec{M}}
\newcommand{\vN}{\myvec{N}}
\newcommand{\vO}{\myvec{O}}
\newcommand{\vP}{\myvec{P}}
\newcommand{\vQ}{\myvec{Q}}
\newcommand{\vR}{\myvec{R}}
\newcommand{\vS}{\myvec{S}}
\newcommand{\vT}{\myvec{T}}
\newcommand{\vU}{\myvec{U}}
\newcommand{\vV}{\myvec{V}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\vX}{\myvec{X}}
%\newcommand{\vXs}{\vX_{\vs}}
\newcommand{\vXs}{\vX_{s}}
\newcommand{\vXt}{\myvec{\tilde{X}}}
\newcommand{\vY}{\myvec{Y}}
\newcommand{\vZ}{\myvec{Z}}


\newcommand{\vxtest}{\myvec{x}_*}
\newcommand{\vytest}{\myvec{y}_*}


\newcommand{\ftrue}{f_{true}}

\newcommand{\myprec}{\mbox{prec}}
\newcommand{\precw}{\lambda_{w}} % precision of weights (alpha)
\newcommand{\precy}{\lambda_{y}} % precision of y (beta)
\newcommand{\fbar}{\overline{f}}
\newcommand{\xmybar}{\overline{x}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\zbar}{\overline{z}}
\newcommand{\vxbar}{\overline{\vx}}
\newcommand{\vXbar}{\overline{\vX}}
\newcommand{\vybar}{\overline{\vy}}
\newcommand{\vYbar}{\overline{\vY}}
\newcommand{\vzbar}{\overline{\vz}}
\newcommand{\vZbar}{\overline{\vZ}}
\newcommand{\xbar}{\overline{x}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\Ybar}{\overline{Y}}
\newcommand{\Gbar}{\overline{G}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Nbar}{\overline{N}}
%\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\Sbar}{\overline{S}}
\newcommand{\vSbar}{\overline{\vS}}
\newcommand{\Rbar}{\overline{R}}

\newcommand{\vtaubar}{\overline{\vtau}}
\newcommand{\vtbar}{\overline{\vt}}
\newcommand{\vsbar}{\overline{\vs}}

\newcommand{\htilde}{\tilde{h}}
\newcommand{\vhtilde}{\tilde{\vh}}
\newcommand{\Dtilde}{\tilde{D}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\wtilde}{\tilde{w}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\pemp}{p_{emp}}
\newcommand{\pstar}{p^*}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\Xtilde}{\tilde{X}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\vxtilde}{\tilde{\vx}}
\newcommand{\vytilde}{\tilde{\vy}}
\newcommand{\ztilde}{\tilde{\z}}
\newcommand{\vztilde}{\tilde{\vz}}
\newcommand{\vthetaMAP}{\hat{\vtheta}_{MAP}}
\newcommand{\vthetaS}{\vtheta^{(s)}}
\newcommand{\vthetahat}{\hat{\vtheta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\overline{\theta}}
\newcommand{\vthetabar}{\overline{\vtheta}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\vpibar}{\overline{\vpi}}


%\newcommand{\subsubsubsection}[1]{\paragraph{#1}}
\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\real}{\mathbb{R}}

\newcommand{\given}{\|}
\newcommand{\indep}[2]{{#1} \perp {#2}}
\newcommand{\condindep}[3]{{#1} \perp {#2} | {#3}}
\newcommand{\condindepG}[3]{{#1} \perp_G {#2} | {#3}}
\newcommand{\condindepP}[3]{{#1} \perp_p {#2} | {#3}}
\newcommand{\depend}[2]{{#1} \not \perp {#2}}
\newcommand{\conddepend}[3]{{#1} \not \perp {#2} | {#3}}

\newcommand{\trans}[1]{{#1}^{\mathtt{T}}}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
%\newcommand{\rv}{r.v.}
\newcommand{\la}{\leftarrow}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\st}{\mbox{  s.t.  }}

\newcommand{\dom}{\mbox{dom}}
\newcommand{\bel}{\mbox{bel}}
\newcommand{\dsep}{\mbox{dsep}}
\newcommand{\sep}{\mbox{sep}}
\newcommand{\entails}{\models}
\newcommand{\range}{\mbox{range}}
\newcommand{\myspan}{\mbox{span}}
\newcommand{\nullspace}{\mbox{nullspace}}
\newcommand{\adj}{\mbox{adj}}

\newcommand{\nbd}{\mbox{nbd}}
\newcommand{\nbr}{\mbox{nbr}}
\newcommand{\anc}{\mbox{anc}}
\newcommand{\desc}{\mbox{desc}}
\newcommand{\pred}{\mbox{pred}}
\newcommand{\nondesc}{\mbox{nondesc}}
\newcommand{\pa}{\pi}
\newcommand{\ch}{\mbox{ch}}
\newcommand{\mb}{\mbox{mb}}
\newcommand{\connects}{\sim}


\newcommand{\betadist}{\mbox{Beta}}
\newcommand{\Betadist}{\mbox{Beta}}
\newcommand{\bernoulli}{\mbox{Ber}}
\newcommand{\Ber}{\mbox{Ber}}
\newcommand{\Binom}{\mbox{Bin}}
\newcommand{\NegBinom}{\mbox{NegBinom}}
\newcommand{\binomdist}{\mbox{Bin}}
\newcommand{\cauchy}{\mbox{Cauchy}}
\newcommand{\DE}{\mbox{DE}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\discrete}{\calM}
\newcommand{\Discrete}{\calM}
\newcommand{\expdist}{\mbox{Exp}}
\newcommand{\expon}{\mbox{Expon}}
\newcommand{\gammadist}{\mbox{Ga}}
\newcommand{\Ga}{\mbox{Ga}}
\newcommand{\gauss}{{\cal N}}
\newcommand{\IG}{\mbox{IG}}
\newcommand{\IGauss}{\mbox{InvGauss}}
\newcommand{\IW}{\mbox{IW}}
\newcommand{\Laplace}{\mbox{Lap}}
\newcommand{\Mu}{\mbox{Mu}}
\newcommand{\Multi}{\mbox{Mu}}
\newcommand{\NIX}{NI\chi^2}
\newcommand{\GIX}{NI\chi^2}
\newcommand{\NIG}{\mbox{NIG}}
\newcommand{\GIG}{\mbox{NIG}}
\newcommand{\NIW}{\mbox{NIW}}
\newcommand{\GIW}{\mbox{NIW}}
\newcommand{\MVNIW}{\mbox{NIW}}
\newcommand{\NW}{\mbox{NWi}}
\newcommand{\MVNIG}{\mbox{NIG}}
\newcommand{\NGdist}{\mbox{NG}}
\newcommand{\prob}{p}
\newcommand{\Poi}{\mbox{Poi}}
\newcommand{\Student}{{\cal T}}
\newcommand{\student}{{\cal T}}
\newcommand{\Wishart}{\mbox{Wi}}
\newcommand{\Wi}{\mbox{Wi}}
\newcommand{\unif}{\mbox{U}}
\newcommand{\etr}{\mbox{etr}}

\newcommand{\softmax}{\calS}
\newcommand{\soft}{\mbox{soft}}
\newcommand{\cond}{\mbox{cond}}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\matlab}{{\sc MATLAB}}
\newcommand{\NETLAB}{{\sc NETLAB}}
\newcommand{\MLABA}{\mbox{PMTK}}
\newcommand{\BLT}{\mbox{PMTK}}
\newcommand{\PMTK}{\mbox{PMTK}}
\newcommand{\mywp}{\mbox{wp}}

\newcommand{\KLpq}[2]{\mathrm{KL}\left[{#1}\|{#2}\right]}
\newcommand{\KL}{\mbox{KL}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MIxy}[2]{\mathbb{I}\left({#1};{#2}\right)}
\newcommand{\MIxyz}[3]{\mathbb{I}\left({#1};{#2}|{#3}\right)}
\newcommand{\entropy}[1]{\mathbb{H}\left({#1}\right)}
\newcommand{\entropypq}[2]{\mathbb{H}\left({#1}, {#2}\right)}


\newcommand{\vvec}{\mbox{vec}}
\newcommand{\kron}{\otimes}
\newcommand{\dof}{\mbox{dof}}
%\newcommand{\E}{E}
\newcommand{\E}{\mathbb{E}}
\newcommand{\energy}{E}
\newcommand{\expectAngle}[1]{\langle #1 \rangle}
%\newcommand{\expect}[1]{\mathbb{E}\left[ {#1} \right]}
\newcommand{\expect}[2]{\mathds{E}_{{#1}} \left[ {#2} \right]}
\newcommand{\expectGiven}[3]{\mathds{E}_{{#1}} \left[ {#2} \mid {#3} \right]}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\VarGiven}[3]{\mbox{Var}_{{#1}}\left[ {#2} \mid {#3}\right]}
%\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}[1]{\mbox{var}\left[{#1}\right]}
\newcommand{\std}[1]{\mbox{std}\left[{#1}\right]}
\newcommand{\varQ}[2]{\mbox{var}_{{#2}}\left[{#1}\right]}
\newcommand{\cov}[1]{\mbox{cov}\left[{#1}\right]}
%\newcommand{\mode}[1]{\mbox{mode}\left[{#1}\right]}
\newcommand{\median}[1]{\mbox{median}\left[{#1}\right]}



\newcommand{\diag}{\mbox{diag}}
\newcommand{\blkdiag}{\mbox{blkdiag}}
\newcommand{\bias}{\mbox{bias}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}

\newcommand{\size}{\mbox{size}}
\newcommand{\trace}{\mbox{trace}}


\newcommand{\myc}{c}
\newcommand{\myi}{i}
\newcommand{\myj}{j}
\newcommand{\myk}{k}
\newcommand{\myn}{n}
\newcommand{\myq}{q}
\newcommand{\mys}{s}
\newcommand{\myt}{t}


\newcommand{\supp}{\mbox{supp}}


\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calDx}{{\cal D}_x}
\newcommand{\calE}{{\cal E}}
\newcommand{\cale}{{\cal e}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calHX}{{\cal H}_X}
\newcommand{\calHy}{{\cal H}_y}
\newcommand{\calI}{{\cal I}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\caln}{{\cal n}}
\newcommand{\calNP}{{\cal NP}}
\newcommand{\calMp}{\calM^+}
\newcommand{\calMm}{\calM^-}
\newcommand{\calMo}{\calM^o}
\newcommand{\Ctest}{C_*}
\newcommand{\calL}{{\cal L}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calq}{{\cal q}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calSstar}{\calS_*}
\newcommand{\calT}{{\cal T}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calv}{{\cal v}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}

\newcommand{\Lone}{$\ell_1$}
\newcommand{\Ltwo}{$\ell_2$}

\newcommand{\mya}{\mbox{a}}
\newcommand{\myat}{\alpha_{t|t-1}}
\newcommand{\score}{\mbox{score}}
\newcommand{\AIC}{\mbox{AIC}}
\newcommand{\BIC}{\mbox{BIC}}
\newcommand{\BICcost}{\mbox{BIC-cost}}
\newcommand{\scoreBIC}{\mbox{score-BIC}}
\newcommand{\scoreBICL}{\mbox{score-BIC-L1}}
\newcommand{\scoreL}{\mbox{score-L1}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mbox{do}}
\newcommand{\data}{\calD}
\newcommand{\model}{\calM}
\newcommand{\dataTrain}{\calD_{\mbox{train}}}
\newcommand{\dataTest}{\calD_{\mbox{test}}}
\newcommand{\dataValid}{\calD_{\mbox{valid}}}
\newcommand{\futuredata}{\tilde{\calD}}
\newcommand{\algo}{\calA}
\newcommand{\fitAlgo}{\calF}
\newcommand{\predictAlgo}{\calP}
\newcommand{\err}{\mbox{err}}
\newcommand{\logit}{\mbox{logit}}
\newcommand{\parent}{\mbox{pa}}


%%%%%%%%%%% Hoyt

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{n}


\newcommand{\condSet}{\mathcal{S}}
\newcommand{\condSetC}{\mathcal{\lnot S}}



==> Cultural General Intelligence (Final Copy for arXiv)/discussion.tex <==
\clearpage
\section{Discussion}
\label{discussion}

\subsection{Summary}

We train an artificial agent capable of robust real-time cultural transmission, and we do so without using human data in the training pipeline. Our work offers the following novel contributions:

\begin{enumerate}
    \item We present a trained neural network solving the full cultural transmission problem, not only inferring information about the task from an expert as in prior work, but also remembering that information within an episode after the expert has dropped out, and leveraging the information to solve hard exploration problems.
    \item We demonstrate that our cultural transmission agent can generalise in few-shot to a wider space of held-out tasks than previously considered, varying the positions of objects in the world, the structure of the game, and the behaviour of the expert player. Moreover, we show that our agent can generalise to cultural transmission from a human expert, a novel step.
    \item Via ablations we identify a minimal sufficient set of ingredients for the emergence of cultural transmission, including several elements which were not previously studied in this context, namely an other-agent attention auxiliary loss, within-episode expert dropout and automatic domain randomisation. 
\end{enumerate} 

\subsection{Commentary}

There are two dual perspectives on open-endedness in RL systems. On the one hand, one can try to construct an agent which has ever increasing reward in a single rich and complex task. On the other, one can try to construct an agent which achieves a reward threshold in an ever more complex space of tasks. In this work, we have found it convenient to take the latter view, because it is more pragmatic for curriculum design. Our agent algorithm itself is surprisingly simple. Perhaps fewer, stronger components is a natural direction of travel when generating more general, social, adaptive agents. We expect that representation learning, scaleable RL algorithms and co-adaptation of training experience will be key for future work in this space. 

We have characterised our approach to generating cultural transmission as memory-based meta-learning. This has several benefits. Imagine deploying a robot in a kitchen. One would hope that the robot would adapt quickly online if the spoons are moved, or if a new chef turns up with different skills. Moreover, one might have privacy concerns about relaying large quantities of data to a central server for training. Our agent adapts to human cultural data online, on-the-fly and within its local memory. It is both robust and privacy-preserving. 

We have shown that social learning research scales to complex $3$-dimensional task distributions. However, we emphasise that scale is not a pre-requisite for a research program on cultural evolution in AI. Indeed, one could implement the same algorithms on a smaller scale and still generate interesting recall and generalisation capabilities across a targeted range of tasks. The fact that we know that the approach scales is useful in motivating further research effort, both small-compute and large-compute. 

\subsection{Limitations}

From a safety perspective, our trained agent as an artefact has a case of objective misgeneralisation \citep{shah2022objective}, which we see in Figure \ref{fig:wrong_demo_trajectory}. The agent happily follows an incorrect demonstration and even reproduces that incorrect path once the expert has dropped out. This is unsurprising since the agent has only encountered near-perfect experts in training. To mitigate this, we hypothesise that an agent should be trained with a variety of experts, including noisy experts and experts with objectives that are different from the agent's. With such experience, an agent should meta-learn a selective social learning strategy \citep{doi:10.1177/0963721415613962, rendell10}, deciding what knowledge to infer from which experts, and when to rely on independent exploration. 

We identify three limitations with our evaluation approach. Firstly, we did not test cultural transmission from a range of humans, but rather with a single player from within the study team. Therefore we cannot make statistically significant claims about robustness across a human population. Secondly, the diversity of reasonable human behaviour is constrained by our navigation task. To gain more insight into generalisable cultural transmission, we need tasks with greater strategic breadth and depth. Lastly, we do not distinguish whether our trained agents memorise a geographical path, or whether they memorise an abstraction over the correct sphere ordering. To disambiguate this, one could change the geographical location of goal spheres at the moment of expert dropout but leave the ordering the same.

Reflecting on whether our method is constrained by our choice of the GoalCycle3D environment, we note that this is already a large, procedurally-generated task space. Moreover, it is the navigational representative for an even bigger class of tasks: those which require a repeated sequence of strategic choices, such as cooking, wayfinding and problem solving. It is reasonable to expect that similar methods would work well in other representative environments from this class of tasks. 

However, there are environmental affordances that we necessarily assume for our method, including expert visibility, dropout and procedural generation. If these are impossible to create or approximate in an environment, then our method cannot be applied. More subtly there are silent assumptions: that finding an initial reward is relatively easy, there is no fine-motor control necessary, the timescale for an episode is relatively short, there are no irreversibilities, the goals are all visible, the rewarding order remains constant throughout an episode. We encourage readers to relax each of these requirements in future work, creating new challenges for research.

Our method is limited in that it requires high-quality co-players for training. We were able to use a hand-coded bot, but this is not typically available in more challenging domains. One potential solution to this problem is to bootstrap agent capabilities across generations using generational training \citep{oelt2021open, vinyals2019grandmaster}. The resulting ratchet effect would lead to agents gradually becoming more capable at cultural transmission. This is a reasonable hypothesis, since cultural transmission can be viewed as amortised distillation, and distillation is already known to work well in generational training. 

\subsection{Future work} 
\label{sec:future_work}

We have focused on the imitation of behaviours. Humans also imitate over more abstract representations of the task at hand, including beliefs, desires and intentions. Whether co-adaptation of training experience can lead to such ``theory of mind'' in artificial agents remains an open question. This approach would complement explicit model-based methods adopted in prior work (e.g. \cite{bratman1987intention, DBLP:journals/corr/abs-1802-07740}).

We motivated this work by observing that cultural transmission is the inheritance process in cultural evolution. In the previous section, we argued that appropriate randomisation over experts may generate a selection process for knowledge. The final missing ingredient for the evolutionary ratchet is variation in behaviour space. Fortunately, there are a variety of off-the-shelf techniques for generating diverse policies \citep{rakicevic2021policy, DBLP:journals/corr/abs-1802-06070, NEURIPS2020_d1dc3a82}. Bringing all of these components together, it would be fascinating to validate or falsify the hypothesis that cultural evolution in a population of agents may yield progressively more generally capable artificial intelligence. 

We do not view our MEDAL-ADR method as a direct model for the development of cultural transmission during human ontogeny. However, the time is ripe for such research. The experimental (e.g. \cite{legare2017cumulative, saldana2019cumulative}) and theoretical (e.g. \cite{tomasello2019becoming, heyes2018cognitive}) fields are already well-developed, and this work provides plausible AI modelling techniques. Neuroscience and deep RL have already mutually benefited from collaborations with a modelling flavour \citep{hassabis2017}, and the precedent has been set for MARL as a modelling tool in social cognition \citep{DBLP:journals/corr/abs-2002-02325, DBLP:journals/corr/abs-2103-04982}. We look forward to fruitful interdisciplinary interaction between the fields of AI and cultural evolutionary psychology in the future. 

==> Cultural General Intelligence (Final Copy for arXiv)/environment.tex <==
\clearpage
\section{Task space}
\label{sec:environment}

To train and evaluate our agents, we introduce a 3D physical simulated task space called \textit{GoalCycle3D}, inspired by the GoalCycle environment of \cite{ndousse2020learning}. This task space allows us to explore cultural transmission of navigational skills: a natural starting point given the importance of navigation in human and animal culture \citep{bond2020wayfinding, jesmer2018ungulate, palacin2011cultural, mueller2013social} and the prior focus on navigation problems in AI \citep{mirowski2016learning, mirowski2018learning, banino2018vector, alonso2020deep}. 

Each task contains procedurally-generated terrain, obstacles, and goal spheres, with parameters randomly sampled on task creation. Each agent is independently rewarded for visiting goals in a particular cyclic order, also randomly sampled on task creation. The correct order is not provided to the agent, so an agent must deduce the rewarding order either by experimentation or via cultural transmission from an expert. Our task space presents navigational challenges of open-ended complexity, parameterised by world size, obstacle density, terrain bumpiness and number of goals. 

\begin{figure}[t]
\centering
\includegraphics[width=1.0\linewidth]{figures/env-at-a-glance.png}
\caption{\small The GoalCycle3D task space at a glance.}
\label{fig:env-at-a-glance}
\end{figure}

Similar to \cite{oelt2021open}, we decompose an agent's task as the direct product of a world, a game and a set of co-players. The world comprises the size and shape of the terrain and locations of objects. The game defines the correct order(s) of goals and the reward dynamics for each player. Co-players are other interactive policies in the world, consuming observations and producing actions. In the remainder of this section, we provide an overview of the world space, game space and player interface, summarised in Figure \ref{fig:env-at-a-glance}. For detailed information, see Appendix \ref{app:task_space}. 
\subsection{World space}\label{sec:world}

Each world is built using the Unity game engine \citep{juliani2018unity, ward2020using}. It is a three-dimensional simulated physical space in which avatars are situated. An avatar is an embodiment of a player in the virtual world and is capable of perception and movement. Each world is perfectly square, of size between $16 \times 16 \SI{}{\meter\squared}$ and $37 \times 37\SI{}{\meter\squared}$. The bumpy terrain is procedurally generated using Libnoise \citep{bevinslibnoise}, parameterised by frequency and amplitude. The playable terrain is bounded by an impermeable barrier, invisible to players but visible to human observers. 

Within the playable terrain are procedurally-generated horizontal and vertical obstacles, parameterised by density. The obstacles create navigational and perception challenges for players. In empty worlds, the path between two goals is often immediately visible, and typically a straight line. In worlds with obstacles, visibility can be highly restricted, since obstacles block vision and the LIDAR sensors used by our agents (see Section \ref{sec:player-interface}). Moreover, players may need to take complex paths to reach a goal, including jumping or crouching, requiring continued actions for many steps. Figures \ref{fig:worlds-same-seed} and \ref{fig:worlds-three-seeds} illustrate some representative worlds using different parameters and seeds.

\subsection{Game space}\label{sec:game}

Players are positively rewarded for visiting \textit{goal} spheres in particular cyclic orders. In each possible order, every goal appears exactly once. Therefore, the set of distinct orders may be conveniently expressed as cyclic permutations of maximum length. To construct a game, given a number of goals $n$, an order $\sigma$ is sampled uniformly at random. The positively rewarding orders for the game are then fixed to be $\{\sigma, \sigma^{-1}\}$ where $\sigma^{-1}$ is the opposite direction of the order $\sigma$. An agent has a chance $\frac{2}{(n-1)!}$ of selecting a correct order at random at the start of each episode. In all our training and evaluation we use $n \geq 4$, so one is always more likely to guess incorrectly. Note that $\sigma$ and $\sigma^{-1}$ are equally difficult, equally rewarding options, provided that the world is not chiral.\footnote{That is to say, assuming there is no difference between the world and its mirror image from above with respect to performing a given trajectory.} 

Players receive a reward of $+1$ for entering a goal in the correct order, given the previous goals entered. The first goal entered in an episode always confers a reward of $+1$. If a player enters an incorrect goal, they receive a reward of $-1$ and must now continue as if this were the first goal they had entered. If a player re-enters the last goal they left, they receive a reward of $0$. The optimal policy is to divine a correct order, by experimentation or observation of an expert, and then visit the spheres in this cyclic order for the rest of the episode. At the start of each episode, goals are placed randomly in the world, subject to the constraint that they do not overlap, achieved via rejection sampling. Figure \ref{fig:goal-cycle-mechs} illustrates some of the game mechanics. 

We can classify paths between goals according to their topology. Distinct topologies are characterised by the number of self-intersections on the path, which we refer to as ``crossings''. Different topologies present players with different challenges, since the relative position of the next goal with respect to the others is altered. Moreover, topologies with a higher number of crossings tend to have longer paths. During training, we use rejection sampling to achieve a uniform distribution over topologies. Figure \ref{fig:game-crossings} depicts all possible topologies in games with 4, 5 and 6 goals, which we refer to as $4$-, $5$-, and $6$-cycle tasks.  

\begin{figure}[htb]
\centering
\includegraphics[width=1.0\linewidth]{figures/games.png}
\caption{An overview of all $4$- $5$-, and $6$-cycle topologies, characterised by the number of crossings in their shortest paths.}
\label{fig:game-crossings}
\end{figure}

\subsection{Player interface}
\label{sec:player-interface}

Human players observe the environment through an egocentric first-person camera with a resolution of $640\times480$ pixels. Agents observe the environment through a LIDAR sensor. The LIDAR sensor performs raycasts uniformly distributed in polar coordinates, with azimuth ranging from $0\degree$ to $360\degree$, altitude ranging from $-90\degree$ to $+90\degree$, and a grid of $14\times 14$ rays. Each ray returns a one-hot encoding of the object with which the ray has intersected (vertical obstacle, horizontal obstacle, goal, avatar, terrain), its distance and, for goals only, its RGB color. The ray only returns the first object with which it collides. Therefore, for agents, all objects are opaque, including goals, and the boundary of the world is invisible. In addition, each agent is equipped with an AVATAR sensor, which outputs the $3$-dimensional relative distance of the nearest co-player in Cartesian coordinates in the frame of reference of the avatar.\footnote{This is used as a regression target during training but not passed as an input to the agent's neural network, so is not required at test time.} Figure \ref{fig:lidar-visualisation} compares the human RGB and agent LIDAR observations.

\begin{figure}[ht]
\centering
\includegraphics[width=1\linewidth]{figures/lidar-visualisation.png}
\caption{(left) A third-person camera view at an instant in time. (centre) The human player RGB observation for the blue avatar. (right) A visualisation of the agent LIDAR observation for the same avatar. Each ray also reports the distance to the hit point, which is not shown in this rendering. The human player observation corresponds approximately to the highlighted central $4\times4$ array of the agent LIDAR observation.}
\label{fig:lidar-visualisation}
\end{figure}

The action space is $5$-dimensional and continuous, with each action dimension taking values in $[-1,1]$. The five dimensions represent moving forwards and backwards, moving left and right, rotating left and right, rotating up and down, and jumping and crouching. Players may take any combination of actions simultaneously. Humans interact using a discretised action set, with each action having values in $\{-1,0,+1\}$, mapped to keyboard inputs. Movement dynamics are subject to inertia: players continue to move in their current direction, albeit at a diminishing rate, even when not sending any movement actions corresponding to that same direction.

Avatars can be controlled by a Unity scripted player, which we dub an \textit{expert bot}. Expert bots are ``oracles'', receiving privileged information about the correct order of goals to traverse, navigating using the Unity NavMesh \citep{vantoll2012}, and jumping and crouching when colliding with horizontal obstacles. These movement patterns are simple heuristics, so the expert bots are not guaranteed to find the most efficient trajectory from one goal to the next. 

\subsection{Probe tasks}\label{sec:probe_tasks}
To better understand and compare the performance of our agents under specific conditions, we test them throughout training on a set of ``probe tasks''. These tasks are hand picked and held out from the training distribution (i.e. they are not used to update any neural network weights). The worlds and games used in our probe tasks are shown in Figure~\ref{fig:probe_tasks}.

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/methods/probes_4.png}
        \caption{\centering Empty world, 4-goal games.}
        \label{fig:probes_simple_4}
    \end{subfigure}
    \hfill
        \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/methods/probes_5.png}
        \caption{\centering Empty world, 5-goal games.}
        \label{fig:probes_simple_5}
    \end{subfigure}
    \begin{subfigure}{0.75\textwidth}
        \includegraphics[width=\textwidth]{figures/methods/probes_complex.png}
        \caption{\centering Complex world, 4- and 5-goal games.}
        \label{fig:probes_complex}
    \end{subfigure}
    \caption{The worlds and games used as probe tasks. These cover a representative range of crossings and colour combinations. The complex world probes require clear examples of jumping behaviours and navigation around vertical obstacles. The human movement pattern in all probes is always goal-directed and near-optimal, but clearly different from a scripted bot, taking some time to get situated in the first few seconds and not taking an identical path on repeated cycles, for instance. See \href{https://sites.google.com/view/dm-cgi\#h.itlel1jrvsnn}{example videos}.
    }
    \label{fig:probe_tasks}
\end{figure}

Importantly, these tasks are not chosen based on agent performance. Instead, they are chosen to represent a wide space of possible worlds, games, and co-players. For example, we desire cultural transmission both in worlds devoid of any obstacles and in worlds that are densely covered. Consequently, we included both in our set of probe tasks. We save checkpoints of agents throughout training at regular intervals and evaluate each checkpoint on the probe tasks. This yields a held-out measure of cultural transmission at different points during training, and is a consistent measure to compare across independent training runs.

While we seek to generate agents capable of robust real-time cultural transmission from human co-players, it is infeasible to measure this during training at the scale necessary for conducting effective research. Therefore we create ``human proxy'' expert co-players for use in our probe tasks as follows. A member of the team plays each task alone and with privileged information about the optimal cycle. For each task, we record the trajectory taken by the human as they demonstrate the correct path. We then replay this trajectory to generate an expert co-player in probe tasks, disabling the human proxy's collision mesh to ensure that the human trajectory cannot be interfered with by the agent under test. 


==> Cultural General Intelligence (Final Copy for arXiv)/evaluation.tex <==
\clearpage

\section{Analysis}
\label{sec:evaluation}

In this section, we analyse our agent. There are three key strands of novelty compared with previous work: strong within-episode recall, generalisation over a diverse task space and rigorous measurement of high-fidelity knowledge transfer. To understand how our agent is capable of this, we ``neuroimage'' the memory activations, finding clearly interpretable individual neurons. We use held-out task seeds in all of our analyses. For full details, see Appendix \ref{app:analysis}.

\subsection{Recall}
To assess the recall capabilities of our agents, we quantify their performance across a set of tasks where the expert drops out. The intuition here is that if our agent is able to recall information well, then its score will remain high for many timesteps even after the expert has dropped out. However, if the agent is simply following the expert or has poor recall, then its score will instead drop greatly.

For each task, we evaluate the score of the agent across a number of contiguous $900$-step trials, comprising an episode of experience for the agent. In the first trial, the expert is present alongside the agent, and thus the agent can infer the optimal path from the expert. However, from the next trial onwards the expert is dropped out, so the agent must continue to solve the task alone. The world, agent, and game are not reset between trial boundaries; we use the term ``trial'' to refer to the bucketing of score accumulated by each player within the time window. We consider recall from two different experts, a scripted bot and a human player. For both, we use the worlds from the 4-goal probe tasks introduced in Section~\ref{sec:probe_tasks}.

Figure~\ref{fig:recall_analysis} compares the recall abilities of our agent trained with expert dropout (MEDAL-ADR) and without (ME–AL, closely related to the prior state of the art in \cite{ndousse2020learning}). Notably, after the expert has dropped out, we see that our MEDAL-ADR agent is able to continue solving the task for the first trial while the ablated ME–AL agent cannot. MEDAL-ADR maintains a good performance for several trials after the expert has dropped out, despite the fact that the agent only experienced $1800$-step episodes during training.

\begin{figure}[htb]
    \centering
    \begin{subfigure}{0.48\textwidth}
         \includegraphics[width=\textwidth]{figures/evaluation/recall_bots.png}
        \label{fig:recall_analysis_bots}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
         \includegraphics[width=\textwidth]{figures/evaluation/recall_humans.png}
        \label{fig:recall_analyis_humans}
    \end{subfigure}    
    \caption{Score of MEDAL-ADR and ME–AL agents across trials since the expert dropped out. (left) The experts are scripted bots. (right) The experts are human trajectories. MEDAL-ADR is able to recall significantly better than ME-AL. An accompanying \href{https://sites.google.com/view/dm-cgi\#h.gjdvzr76oj4x}{video} shows MEDAL-ADR's memorisation in a $3600$-step ($4$ trial) episode.}
    \label{fig:recall_analysis}
\end{figure}

\subsection{Generalisation}
To assess the generalisation capabilities of our agents, we quantify their performance over a distribution of procedurally-generated tasks. We decompose our analysis of generalisation into world space, game space, and expert space. We analyse both ``in-distribution'' and ``out-of-distribution'' generalisation, with respect to the distribution of parameters seen in training (see Table~\ref{tab:adr-parameters-id-ood}). Out-of-distribution values are calculated as $\pm$20\% of the min/max in-distribution ADR values where possible, and indicated by cross-hatched bars in all figures. 

In every task, an expert bot is present for the first $900$ steps, and is dropped out for the remaining $900$ steps. We define the \textit{normalised score} as the agent's score in $1800$ steps divided by the expert's score in $900$ steps. An agent which can perfectly follow but cannot remember will score $1$. An agent which can perfectly follow and can perfectly remember will score $2$. Values in between correspond to increasing levels of cultural transmission.

\paragraph{World space} The space of worlds is parameterised by the size and bumpiness of the terrain (terrain complexity) and the density of obstacles (obstacle complexity). To quantify generalisation over this space, we generate tasks with worlds from the Cartesian product of these complexities, with zero-noise expert bots, and with games uniformly sampled across the possible number of crossings for 5 goals. 

\begin{figure}[htb]
    \centering
    \begin{subfigure}{0.48\textwidth}
         \includegraphics[width=\textwidth]{figures/evaluation/generalization_world_space.png}
        \caption{\centering Normalised score across complexities.}
        \label{fig:generalization-analysis-world-space-score}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
         \includegraphics[width=\textwidth]{figures/evaluation/generalization_world_space_examples.png}
        \caption{\centering Example worlds sampled from the extremal values of the distribution parameters.}
        \label{fig:generalization-analysis-world-space-example}
    \end{subfigure} 
    \caption{MEDAL-ADR generalises across world space parameters, demonstrating both following and remembering across much of the space. Obstacle complexity and terrain complexity are defined in Appendix \ref{app:analysis}. Hatched cells denote out-of-distribution values. Sample videos for the extremal values can be found on the  \href{https://sites.google.com/view/dm-cgi\#h.ms6jr5zahrco}{website}.}
    \label{fig:generalization-analysis-world-space}
\end{figure}

\begin{figure}[htb]
    \centering
     \includegraphics[scale=0.35]{figures/evaluation/generalization_world_space_1d_top.png}
     \includegraphics[scale=0.35]{figures/evaluation/generalization_world_space_1d_bottom.png}     
    \caption{A slice through the world space allows us to disentangle MEDAL-ADR's generalisation capability across different world space parameters. For the top parameters (terrain complexity), larger values lead to a gradual reduction in performance. For the bottom parameters (obstacle complexity), performance is stable until they reach their larger out-of-distribution values.}
    \label{fig:generalization-analysis-world-space-individual}
\end{figure}

From Figures \ref{fig:generalization-analysis-world-space} and \ref{fig:generalization-analysis-world-space-individual}, we conclude that MEDAL-ADR generalises well across the space of worlds, demonstrating both following and remembering across a majority of the space, including when the world is out-of-distribution. As both obstacle and terrain complexity increases, the performance of our agent drops. For example, as both complexities exceed 0.8 (and are therefore out-of-distribution), the agent's score drops below 1: while it can follow near-perfectly, it is unable to remember. Score gradually decreases as each of the world's individual parameters increases. This is most notable with the world size parameter. Comparing to Figure \ref{fig:adr-full-training}, this is unsurprising: it is likely that a combination of more training, a longer recurrent unroll, and a larger memory may be required to generate an agent capable of cultural transmission in larger worlds, where the number of timesteps for a complete goal cycle demonstration is larger.

\paragraph{Game space} The space of games is defined by the number of goals in the world as well as the number of crossings contained in the correct navigation path between them. To quantify generalisation over this space, we generate tasks across the range of feasible ``$N$-goal $M$-crossing'' games, each with a zero-noise expert bot in a flat empty world of size 23.

Figure~\ref{fig:generalization-analysis-task-space} shows our agent's ability to generalise across games, including those outside of its training distribution. Notably, MEDAL-ADR can perfectly remember all numbers of crossings for the in-distribution 5-goal game. We also see impressive out-of-distribution generalisation, with our agent exhibiting strong remembering, both in $4$-goal and $0$-crossing $6$-goal games. Even in complex $6$-goal games with many crossings, our agent can still perfectly follow. Clearly we require more randomisation to get good generalisation of memorisation to higher numbers of goals.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/evaluation/generalization_game_space.png}
    \caption{MEDAL-ADR generalises across games, demonstrating remembering capability both inside and outside the training distribution. Hatched bars denote out-of-distribution values. This can be seen in the \href{https://sites.google.com/view/dm-cgi\#h.xfaxoqy5f3ls}{videos} of generalisation over the game space.}
    \label{fig:generalization-analysis-task-space}
\end{figure}

\paragraph{Expert space} The space of experts is defined by the speed, dropout probability, and action distribution taken by the expert in the world. To quantify generalisation over this space, we generate tasks with expert bots from the Cartesian product of movement speed and dropout probability, flat empty worlds of size 23, and games uniformly sampled across the possible number of crossings for 5-goals.

Figure~\ref{fig:generalization-analysis-expert-space} demonstrates that MEDAL-ADR generalises well across a range of speeds and dropout probabilities, with consistent remembering of demonstrated trajectories. Furthermore, we can see that our agent is also robust to the introduction of noise in the expert's movement, exhibiting the ability to divine and recall the optimal path until the noise exceeds 30\% and succeeding at the task before dropout by following even with 50\% noise (despite never experiencing expert noise in training). Above 50\% noise, the expert's policy becomes degenerate and therefore unusable for solving the task.

\begin{figure}[htb]
    \centering
    \begin{subfigure}{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/evaluation/generalization_expert_space.png}
        \label{fig:generalization-analysis-expert-space-3d}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.48\textwidth}
         \includegraphics[width=\textwidth]{figures/evaluation/generalization_expert_space_noise.png}
        \label{fig:generalization-analysis-expert-space-noise}
    \end{subfigure} 
    \caption{Influence of variation in expert's parameters on MEDAL-ADR's performance. MEDAL-ADR generalises when paired with a variety of expert co-players (left), and is robust to significant levels of out-of-distribution noise in their movement (right). Normalisation in both plots is done with respect to the non-noisy expert bot with a speed of 13, for interpretability independent of the quality of the expert. In all episodes the bot drops out fully after $900$ steps. Videos of these episodes can be found on the \href{https://sites.google.com/view/dm-cgi\#h.ltw8sokd3hnk}{microsite}.}
    \label{fig:generalization-analysis-expert-space}
\end{figure}

\subsection{Fidelity}
\label{sec:fidelity}

\cite{Dawson1965ObservationalLI} introduced the ``two-action task'' as a means by which to study imitation of behaviours. In this experimental set-up, subjects are required to solve a task with two alternative solutions. Half of the subjects observe a demonstration of one solution, the others observe a demonstration of the other solution. If subjects disproportionately use the observed solution, this is evidence that supports imitation. This experimental approach is widely used in the field of social learning; we use it as a behavioural analysis tool for artificial agents for the first time, to our knowledge. Using the tasks from our game space analysis, we record the preference of the agent in pairs of episodes where the expert demonstrates the optimal cycles $\sigma$ and $\sigma^{-1}$. The preference is computed as the percentage of correct complete cycles that an agent completes which match the direction of the expert cycle. Evaluating this over 1000 trials, we find that the agent's preference matched the demonstrated option $100\%$ of the time, i.e. in every completed cycle of every one of the $1000$ trials.

Trajectory plots reveal the correlation between expert and agent behaviour (see Figure \ref{fig:trajectory_plots}). By comparing trajectories under different conditions, we can argue that cultural transmission of information from expert to agent is causal. The agent cannot solve the task when the bot is not placed in the environment (Figure~\ref{fig:no_bot_trajectory}). When the bot is placed in the environment, the agent is able to successfully reach each goal (Figure \ref{fig:wrong_bot_trajectory}). Even when the bot begins performing incorrectly halfway through the episode, the agent continues to follow (Figure \ref{fig:wrong_bot_trajectory}). However, the agent is not dependent on the bot's continual presence. When the bot drops out, the agent continues to execute the demonstrated trajectory, whether right (Figure \ref{fig:dropout_trajectory}) or wrong (Figure \ref{fig:wrong_demo_trajectory}). 

\begin{figure}[htb]
    \centering
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{figures/trajectories/no_bot.png}
        \caption{\centering The bot is absent for the whole episode.}
        \vspace{1cm}
        \label{fig:no_bot_trajectory}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{figures/trajectories/wrong_trajectory_bot.png}
        \caption{\centering The bot shows a correct trajectory for $900$ steps followed by an incorrect trajectory.}
        \vspace{1cm}
        \label{fig:wrong_bot_trajectory}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{figures/trajectories/dropout_bot.png}
        \caption{\centering The bot shows a correct trajectory in the first half of the episode and then drops out.}
        \vspace{1cm}
        \label{fig:dropout_trajectory}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{figures/trajectories/wrong_demo.png}
        \caption{\centering The bot shows an incorrect trajectory in the first half of the episode and then drops out.}
        \label{fig:wrong_demo_trajectory}
    \end{subfigure}
    \caption{Trajectory plots for MEDAL-ADR agent for a single episode. The coloured parts of the lines correspond to the colour of the goal sphere the agent and expert have entered and the $\times$s correspond to when the agent entered the incorrect goal. Here, position refers to the agent's position along the z-axis. Four corresponding \href{https://sites.google.com/view/dm-cgi\#h.mbxtqto8j9b2}{videos} are available.}
    \label{fig:trajectory_plots}
\end{figure} 

\subsection{Neural activations}

Here, we ``neuroimage'' our agents to gain insights into the specific information represented by neurons in the belief state representation. We find two types of neurons with specialised roles: one, dubbed the \textit{social neuron}, encapsulates the notion of agency; the other, called a \textit{goal neuron}, captures the periodicity of the task. 

A social neuron crisply encodes the presence or absence of the expert in the world. We detect such neurons using a linear probing method \citep{alain2016understanding, anand2019unsupervised} described in Appendix \ref{app:bonus-neural-activations}. This stark difference between the three agents probed in Figure \ref{fig:social-neuron-accuracy} suggests that the attention loss is (at least partly) responsible for incentivising the construction of ``socially-aware'' representations. Qualitatively, Figure \ref{fig:social-neuron-activations} shows that the activations of the maximally weighted neurons have meaningfully different magnitudes and opposing signs depending on whether the expert is present or not.

\begin{figure}[tbp]
    \centering
    \begin{subfigure}[b]{0.47\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures/activations/social-neuron-accuracy.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.47\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/activations/activations-social-neuron-47-medal-adr.png}
        \label{subfig:medal-adr-activations}
    \end{subfigure}
    \caption{(left) We report the accuracy of three models for predicting the expert's presence based on the belief states of three trained agents (MED––, MEDAL, and MEDAL-ADR). We make two causal interventions (in green and purple) and a control check (in red) on the original test set (yellow). The small error bars, drawn from 10 different initialisation seeds, suggest a widespread consensus across the 10 runs on which neurons are social and how impactful they are on task performance. (right) Activations for one of MEDAL-ADR's social neurons.}
\label{fig:social-neuron-accuracy}
\end{figure}

The activation of a goal neuron is highly correlated with the entry of an agent into a goal sphere. We identified a goal neuron by inspecting the variance of belief state neural activations across an episode. Figure \ref{fig:cyclic-neuron-with-sphere-shading} shows that this neuron fires when the agent enters and remains within a goal sphere. For further empirical observations about the goal neuron, see Appendix \ref{app:bonus-attention-loss}.

\begin{figure}[htb]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \includegraphics[width=\textwidth]{figures/activations/cyclic_neuron_full_bot.png}
        \caption{\centering Perfect bot for the entire episode.}
        \label{subfig:cyclic-neuron-full}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/activations/cyclic_neuron_no_bot.png}
        \caption{\centering No bot for the entire episode.}
        \label{subfig:cyclic-neuron-no-bot}
    \end{subfigure}
    
    \vspace{2mm}
    
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/activations/cyclic_neuron_half_bot.png}
        \caption{\centering Perfect bot drops out after half of the episode.}
        \label{subfig:cyclic-neuron-half}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/activations/cyclic_neuron_noisy_bot.png}
        \caption{\centering Noisy bot for the entire episode.}
        \label{subfig:cyclic-neuron-noisy}
    \end{subfigure}
    \caption{Spikes in the goal neuron's activations correlate with the time the agent remains inside a goal (illustrated by coloured shading), irrespective of the reward received.}
\label{fig:cyclic-neuron-with-sphere-shading}
\end{figure}

==> Cultural General Intelligence (Final Copy for arXiv)/introduction.tex <==
\leavevmode\newpage
\section{Introduction}
\label{sec:introduction}

Intelligence can be defined as the ability to acquire new knowledge, skills, and behaviours efficiently across a wide range of contexts \citep{chollet2019measure}. Human intelligence is especially dependent on our ability to acquire knowledge efficiently from other humans. This knowledge is collectively known as culture, and the transfer of knowledge from one individual to another is known as \emph{cultural transmission}. Cultural transmission is a form of social learning, learning assisted by contact with other agents. It is specialised for the inheritance of culture \citep{heyes2018cognitive} via high fidelity, consistent recall, and generalisation to previously unseen situations. We refer to these properties as \textit{robustness} \citep{marcus2020next}. Robust cultural transmission is ubiquitous in everyday human social interaction, particularly in novel contexts: copying a new recipe as seen on TV, following the leader on a guided tour, showing a colleague how the printer works, and so on. 

We seek to generate an artificially intelligent agent capable of robust real-time cultural transmission from human co-players in a rich 3D physical simulation. The motivations for this are threefold. First, since cultural transmission is an ever-present feature of human social behaviour, it is a skill that an artificially intelligent agent should possess to facilitate beneficial human-AI interaction. Second, cultural transmission is the inheritance process that underlies the (Darwinian) evolution of culture \citep{blackmore2000meme},\footnote{Cultural evolution, like all evolution by natural selection, is the inevitable consequence of three processes: variation, selection and inheritance.} arguably the fastest known intelligence-generating process \citep{henrich2015secret}. A convincing demonstration of cultural transmission would pave the way for cultural evolution as an AI-generating algorithm \citep{clune2019ai, leibo2019autocurricula}. Third, rich 3D physical simulations with sparse reward pose hard exploration problems for artificial agents, yet human behaviour in this setting is often highly informative and cheap in small quantities. Cultural transmission provides an efficient means of structured exploration in behaviour space.

We focus on a particular form of cultural transmission, known in the psychology and neuroscience literature as observational learning \citep{bandura1977social} or imitation \citep{heyes2016homo}. In this field, imitation is defined to be the copying of body movement. It is a particularly impressive form of cultural transmission because it requires solving the challenging ``correspondence problem'' \citep{nehaniv2002correspondence}, instantaneously translating a sensory observation of another agent's motor behaviour into a motor reproduction of that behaviour oneself. In humans, imitation provides the kind of high-fidelity cultural transmission needed for the cultural evolution of tools and technology \citep{de1903laws, meltzoff1988imitation}. Borrowing the language of cognitive science, we want to know how the skill of cultural transmission can develop during artificial agent ontogeny, or more colloquially, childhood \citep{tomasello2016ontogeny}.

Our artificial agent is parameterised by a neural network and we use deep reinforcement learning (RL) to train the weights. The resulting neural network (with fixed weights) is capable of zero-shot, high-recall cultural transmission within a ``test'' episode on a wide range of previously unseen tasks. Our approach contrasts with prior methods in which the training itself is a process of cultural transmission, namely imitation learning \citep{argall2009survey, hussein2017imitation, edwards2019imitating, torabi2019recent} and policy distillation \citep{hinton2015distilling, rusu2016policy}. These methods are highly effective on individual tasks, but they are not few-shot learners, require privileged access to datasets of human demonstrations or a target policy, and struggle to generalise to held-out tasks \citep{ren2020generalization}. Closer to our setting, \cite{borsa2017observational,woodward2020learning,ndousse2020learning} use RL to generate test-time social learning, but these agents lack the ability of within-episode recall and only generalise across a limited task space. 

\clearpage
The central novelty in this work is the application of agent-environment co-adaptation \citep{wang2019paired, oelt2021open} to generate an agent capable of robust real-time cultural transmission. To this end, we introduce a new open-ended reinforcement learning environment, \textit{GoalCycle3D}. This environment offers a diverse task space by virtue of procedural generation, 3D rigid-body physics, and continuous first-person sensorimotor control. Here, we explore more challenging exploration problems and generalisation challenges than in previous literature. We introduce a rigorous \textit{cultural transmission metric} and transplant a two-option paradigm from cognitive science \citep{Dawson1965ObservationalLI,whiten1998imitation, aplin2015experimentally} to make causal inference about information transfer from one individual to another. This puts us on a firm footing from which to establish state-of-the-art generalisation and recall capabilities.

Via careful ablations, we identify a minimal sufficient ``starter kit'' of training ingredients required for cultural transmission to emerge, namely function approximation, memory (M), the presence of an expert co-player (E), expert dropout (D), attentional bias towards the expert (AL), and automatic domain randomisation (ADR). We refer to this collection by the acronym MEDAL-ADR. Individually, these components aren't complex, but together they generate a powerful agent. We analyse the capabilities and limitations of our agent's cultural transmission abilities on three axes inspired by the cognitive science of imitation, namely recall, generalisation, and fidelity. We find that cultural transmission generalises outside the training distribution, and that agents recall demonstrations within a single episode long after the expert has departed. Introspecting the agent's "brain", we find strikingly interpretable neurons responsible for encoding social information and goal states. 


==> Cultural General Intelligence (Final Copy for arXiv)/methods.tex <==
\clearpage
\section{Methods}
\label{sec:training}

Here we describe the minimal sufficient list of ingredients for the emergence of robust real-time cultural transmission. Individually, none of the ingredients are complex. Yet, from these simple, general building blocks arises an agent with powerful generalisation and recall. 

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/method_overview.png}
    \caption{The minimal sufficient ingredients that comprise our methods, grouped by the timescale on which they operate.}
    \label{fig:method-overview}
\end{figure}

\subsection{Cultural Transmission (CT) metric}\label{sec:ctmetric}

To rigorously evaluate the cultural transmission capability of a fixed neural network, we must first define precisely what this means. Na\"ively, the agent must improve its performance upon witnessing an expert demonstration, and maintain that improvement within the same episode once the demonstrator has departed. But this is not quite a sufficient condition, for two reasons. 

First, what seems like test-time cultural transmission might actually be cultural transmission during training, leading to memorisation (and subsequent deployment) of fixed navigation routes. To address this, we evaluate cultural transmission in held-out test tasks and with human expert demonstrators \citep{cobbe2020leveraging, anand2021procedural, justesen2018illuminating}, similar to the familiar train-test dataset split in supervised learning \citep{xu2018splitting}. Capturing this intuition, we define a scalar \textit{cultural transmission metric} below. 

Second, what looks like test-time cultural transmission may in fact merely be independent behaviour, conditioned on the presence of a co-player, but not the information they bear. To address this, we borrow the ``two-option paradigm'', standard in studies of animal imitation \citep{Dawson1965ObservationalLI,whiten1998imitation, aplin2015experimentally}. Every one of our tasks contains two different, equally difficult, and equally rewarding options, of which the expert demonstrates only one. We find that our agent consistently displays the same option as the expert, both when together with the expert and after the expert has dropped out. This provides evidence of test-time cultural transmission (see Section \ref{sec:fidelity}). Crucially, there is no option bias during training or testing: in any given task we sample the expert's direction uniformly at random from the $2$ optimal possibilities. 

Let $E$ be the total score achieved by the expert in an episode of a given task. Let $A_{\text{full}}$ be the score of an agent with the expert present for the full episode. Let $A_{\text{solo}}$ be the score of the same agent without the expert. Finally, let $A_{\text{half}}$ be the score of the agent with the expert present from the start to halfway into the episode. These tasks are implemented by using the expert dropout types `No', `Full', and `Half', described in Section~\ref{sec:expert_dropout}. We define the cultural transmission (CT) metric as

\begin{equation}\label{eqn:ctmetric}
    \textrm{CT} \defeq \frac{1}{2}\frac{A_{\text{full}} - A_{\text{solo}}}{E} + 
    \frac{1}{2}\frac{A_{\text{half}} - A_{\text{solo}}}{E} \, .
\end{equation}

We identify several important values for CT. A completely independent agent doesn't use any information from the expert. Therefore it has a value of CT near $0$, since $A_{\text{full}}$, $A_{\text{solo}}$, and $A_{\text{half}}$ are all similar. A fully expert-dependent agent has a value of CT near $0.75$. This is because $A_{\text{full}} \approx E$, $A_{\text{solo}}\approx 0$ and $A_{\text{half}}\approx 0.5 E$, making the first term close to $0.5$ and the second term close to $0.25$. An agent that follows perfectly when the expert is present, but continues to achieve high scores once the expert is absent has a value of CT near $1$. This is the desired behaviour of an agent from a cultural transmission perspective, since the knowledge about how to solve the task was transmitted to, retained by and reproduced by the agent. Note that CT does not distinguish well between perfect following and the combination of imperfect following and imperfect recall. This motivates the more detailed analysis of our agent's capabilities in Section \ref{sec:evaluation}.

\subsection{Agent architecture and Memory (M)}

Our agent architecture is depicted in Figure \ref{fig:agent-architecture}. The encoded observation is fed to a single-layer recurrent neural network (RNN) with an LSTM core \citep{hochreiter1997lstm} of size $512$. This RNN is unrolled for $800$ steps during training. The output of the LSTM, which we refer to as the \textit{belief}, is passed to a policy, value and auxiliary prediction head. The policy and value heads together implement the MPO algorithm, while the prediction head implements the attention loss described in Section \ref{sec:auxloss}. The AVATAR sensor observation is used as a prediction target for this loss. Our agent is trained using a large scale distributed training framework, described in Appendix \ref{sec:training-framework}. Further details of the hyperparameters used for learning are reported in Appendices
\ref{sec:hyperparameters}.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/agent_architecture.png}
    \caption{Agent architecture, including training losses.}
    \label{fig:agent-architecture}
\end{figure}

\subsection{Expert Dropout (ED)}\label{sec:expert_dropout}

Cultural transmission requires the acquisition of new behaviours from others. For an agent to robustly demonstrate cultural transmission, it is not sufficient to imitate instantaneously; the agent must also internalise this information, and later recall it in order to display the transmitted behaviour. We introduce \textit{expert dropout} as a mechanism both to test for and to train for this recall ability. 

At each timestep in an episode, the expert is rendered visible or hidden from the agent. Given a difficult exploration task which the agent cannot solve through solo exploration, we can measure its ability to recall information gathered through cultural transmission by observing whether or not it is able to solve the task during the contiguous steps in which the expert is hidden. During training, we apply expert dropout in an automatic curriculum to encourage this recall ability, as described in Section \ref{sec:adr}.

Mathematically, we formulate expert dropout as follows. Let $e_t \in \mathbb{Z}_2$ be the \emph{state} of expert dropout at timestep $t$. State $0$ corresponds to the expert being hidden at time $t$, by which we mean it will not be detected in any player's observation. State $1$ corresponds to the expert being visible at time $t$. An expert dropout scheme is characterised by the state transition functions $e_{t+1} = f(e_t, t)$. We define the following schemes:
\begin{multicols}{2}
\paragraph{No dropout} $f(e_t, t) = 1$ for all $t$.
\columnbreak
\paragraph{Full dropout} $f(e_t, t) = 0$ for all $t$.
\end{multicols}
\paragraph{Half dropout} For episodes of length $N$ timesteps, 
\begin{equation}
f(e_t, t) = 
\begin{cases}
1 & t \leq \lfloor N/2 \rfloor \\
0 & t > \lfloor N/2 \rfloor \\
\end{cases}.
\end{equation}

\paragraph{Probabilistic dropout} Given transition probability $p \in [0, 1]$,
\begin{equation}
    f(e_t, t) = 
    \begin{cases}
    e_t + 1 \mod 2& \text{with probability $p$} \\
    e_t & \text{with probability $1 - p$} \\
    \end{cases}.
\end{equation}

\subsection{Attention Loss (AL)}\label{sec:auxloss}

To use social information, agents need to notice that there are other players in the world that have similar abilities and intentions as themselves \citep{ndousse2020learning, DBLP:journals/corr/abs-1802-07740}. Agents observe the environment without receiving other players' explicit actions or observations, which we view as privileged information. Therefore, we propose an \textit{attention loss} which encourages the agent's belief to represent information about the current relative position of other players in the world. We use ``attention'' here in the biological sense, identifying what is important, in particular, that agents should pay attention to their co-players. Similar to previous work (e.g. \citet{DBLP:journals/corr/abs-1906-01470}), we use a privileged AVATAR sensor as a prediction target, but not as an input to the neural network, so it is not required at test time. 

Starting from the belief, we concatenate the agent's current action, pass this through two MLP layers of size $32$ and $64$ with \textit{relu} activations, and finally predict the egocentric relative position of other players in the world at the current timestep. The objective is to minimise the $\ell^1$ distance between the ground truth and predicted relative positions. The attention loss is set to zero when the agent is alone (for instance, when the expert has dropped out). For more details, including empirical determination of attention loss hyperparameters, see Appendix \ref{app:bonus-attention-loss}.

\subsection{Automatic Domain Randomisation (ADR)}\label{sec:adr}

An important ingredient for the development of cultural transmission in agents is the ability to train over a diverse set of tasks. Without diversity, an agent can simply learn to memorise an optimal route. It will pay no attention to an expert at test-time and its behaviour will not transfer to distinct, held-out tasks. This diverse set of tasks must be adapted according to the current ability of the agent. In humans, this corresponds to Vygotsky's concept of a dynamic ``Zone of Proximal Development'' (ZPD). \citep{vygotsky1980mind}. This is defined to be the difference between a child's ``actual development level as determined by independent problem solving'' and ``potential development as determined through problem solving under adult guidance or in collaboration with more capable peers''. We also refer to the ZPD by the more colloquial term ``Goldilocks zone'', one where the difficulty of the task is not too easy nor too hard, but just right for the agent.

We use Automatic Domain Randomisation (ADR) \citep{openai2019} to maintain task diversity in the Goldilocks zone for learning a test-time cultural transmission ability. To apply ADR, each task must be parameterised by a set of $d$ parameters, denoted by $\lambda \in \mathbb{R}^d$. In \textit{GoalCycle3D}, these parameters may be related to the world, such as terrain size or tree density, the game, such as number of goals, or the co-players, such as bot speed.

Each set of task parameters $\lambda$ are drawn from a distribution $P_{\phi}(\Lambda)$ over the $(d-1)$-dimensional standard simplex, parameterised by a vector $\phi$. We use a product of uniform distributions with $2d$ parameters and joint cumulative density function
\begin{equation}
P_{\phi}(\lambda) = \prod_{i=1}^d \frac{1}{\phi_i^L - \phi_i^H} \, ,
\end{equation}
defined over the standard simplex given by 
\begin{equation}
\left\{
\lambda: \lambda_i \in [\phi_i^L,\, \phi_i^H] \text{ for } 
i \in \{1,\dots,d\}\text{, }
\lambda \in \mathbb{R}^d
\right
\} \, .
\end{equation}

Roughly speaking, the simplex boundaries $\phi_{i}^L$ or $\phi_{i}^H$ are expanded if the training cultural transmission metric exceeds an upper threshold and contracted if the training cultural transmission metric drops below a lower threshold. This maintains the task distribution in the Goldilocks zone for learning cultural transmission. For more details, see Appendix \ref{sec:app_adr}.

==> Cultural General Intelligence (Final Copy for arXiv)/related_work.tex <==
\clearpage
\section{Related work}
\label{sec:related_work}

Our work continues a long line of research about how to generate artificial agents that imitate human behaviour online in rich 3D physical environments, most prominently in the robotics community (see \cite{BREAZEAL2002481} for a review). Much of this work has employed model-based systems to make online learning sample efficient (e.g. \cite{614389}), sometimes taking inspiration from prediction mechanisms in the human brain (e.g. \cite{doi:10.1080/09540090310001655129, 6789045}). Inspired by this, we ask whether it is possible to use model-free RL to learn an implicit model in the memory of a neural network, which at test-time is capable of online imitation. The answer is ``yes''. Our approach inherits the scaleability advantages of model-free methods \citep{DBLP:journals/corr/abs-1806-02308}, but retains the sample-efficiency of model-based methods at test time. Because our method makes heavy use of domain randomisation, it may even be amenable to use in sim-to-real contexts \citep{DBLP:journals/corr/abs-2010-11251}. 

Previous works have used model-free reinforcement learning to generate a fixed policy capable of test-time social learning and generalisation to held out tasks. \cite{borsa2017observational} demonstrated that A3C agents \citep{mnih2016asynchronous} were capable of learning to find and follow an expert co-player in a grid-world navigation task, purely on the basis of goal-location reward. Agents trained on a four-room maze generalised in zero-shot to follow in a nine-room maze. When the presence of the expert was dropped out across training, the agent learned to solve the nine-room maze fully independently. However, the authors did not produce a fixed policy capable of reproducing a demonstrated trajectory after expert dropout within a single evaluation episode.

\cite{ndousse2020learning} extend the work of \cite{borsa2017observational}, demonstrating more rigorously that learning social learning improves generalisation to held-out tasks and achieves better performance than solo baselines on hard exploration problems. Crucial to the success of their agents is a next-step prediction auxiliary loss \citep{shelhamer2016loss, jaderberg2016reinforcement}. The authors introduce the \textit{GoalCycle} environment where task knowledge comprises navigating goals in the correct order, in principle providing parameterised, open-ended navigational complexity. Similarly to previous work, \cite{ndousse2020learning} do not generate an agent capable of within-episode recall. 

There have been various works leveraging reinforcement learning to generalise to human co-play in coordination tasks, without using human data in the training pipeline. FCP \citep{strouse2021fcp} uses a population of self-play agents and their past checkpoints as a training distribution for a focal agent in a grid-world version of Overcooked \citep{carroll2019utility}, producing agents that generalise well to human co-play on the same task seen in training. LILA \citep{woodward2020learning} uses multi-agent deep RL to generate an agent capable of inferring a ``principal'' agent's goal, namely the preference for one of two object types, and using this information to assist the principal, achieve good performance with human co-players in simple grid-worlds. We take inspiration from these works, but tackle a different problem: high fidelity cultural transmission of long, strategic behaviours.

A line of work in the card game Hanabi \citep{bard2020hanabi} is also oriented in this direction, generating zero-shot coordination with human players via various explicit modelling techniques, including by exploiting symmetries \citep{hu2020other, bullard2021quasi}, learned belief search \citep{hu2021learned}, diversity algorithms \citep{canaan2020generating, lupu2021trajectory} and modelling theory of mind \citep{zhu2021few}. Hanabi is a turn-based game in which all actions are visible and each player has different legal actions, so it is not an appropriate arena in which to study the correspondence problem. 

We identify a minimal sufficient ``starter kit'' of ingredients (MEDAL-ADR) that give rise to a fixed neural network capable of cultural transmission. Many of these ingredients build off prior work. The importance of memory (M) was already identified via ablations in \citep{borsa2017observational}, and echoes the presence of recurrent state in meta-RL algorithms \cite{wang2016learning, duan2016rl}. Theoretically, our setting is automatically a POMDP, since the policy of the expert and the details of the task sampling are hidden information. Therefore, we would expect memory to be essential in de-aliasing states via observation of task dynamics and expert behaviour over time \citep{wierstra2007solving}. The presence of expert co-players (E) was already ablated in \citep{borsa2017observational}; we provide additional ablations that explore how the reliability of the expert affects the learning of cultural transmission, inspired by the competence dimension of interpersonal perception \citep{fiske2002model}. 

Dropout (D) is a well studied mechanism for reducing overfitting in many fields of machine learning \citep{labach2019survey}, and was used across training episodes in \cite{borsa2017observational, ndousse2020learning}. To our knowledge, we are the first to use co-player dropout \textit{within} the course of an episode. 

Unsupervised auxiliary losses in reinforcement learning were introduced in \cite{jaderberg2016reinforcement}, and are commonly used to shape representations, promoting more efficient learning, and helping to overcome hard exploration problems. \cite{ndousse2020learning} found that a next-step prediction loss was beneficial to promote social learning in a grid-world setting. Reconstruction losses in particular tend to have beneficial effects on generalisation \citep{le2018supervised}. We use a novel unsupervised auxiliary reconstruction loss focused on the relative position of co-players, which we refer to as an attention loss (AL).  

Automatic domain randomisation (ADR) is a technique within the broader field of co-adaptation of agents and environments to yield generalisation. Its precursor, domain randomisation (DR), used uniform sampling of a diverse set of environments and tasks to bridge the sim-to-real gap in robotics~\cite{peng2017domainrandomization, tobin2017domainrandomization}. ADR extended DR by automatically adapting the randomisation ranges to agent performance, leading to the zero-shot transfer of a policy for a complex, in-hand manipulation task from simulation to a real-world robot~\cite{openai2019}. Other forms of agent-environment co-adaptation include \cite{everett2019optimising, wang2019paired, DBLP:journals/corr/abs-2110-02439}. In the multi-agent setting, agent-agent interactions provide a rich source of autocurricula \citep{DBLP:journals/corr/abs-2012-02096, leibo2019autocurricula, DBLP:journals/corr/abs-1909-07528, oelt2021open} in which co-operation and competition can scale the task difficulty automatically as agents become more capable.

All of these ingredients have analogues in human and animal cognition. Better working memory (M) is known to correlate with improved fluid intelligence in humans \citep{duncan2012task} and the ability to solve novel reasoning problems \citep{cattell1963theory}, including by imitation \citep{vostroknutov2018role}. The quality of expert demonstrations (E) is a crucial determinant of the success of cultural transmission in humans, to the extent that humans possess psychological adaptations to enhance quality when multiple models are available, such as prestige bias \citep{henrich2001evolution}. 

The progressive increase in duration of expert dropout (D) mirrors the development of secure attachment in attachment theory \citep{bowlby1958nature, harlow1958nature}, where a human child learns to use their caregiver as a safe base for independent behaviour when that caregiver is absent. The success of expert dropout as a means of learning to recall demonstrations across contexts echoes the discovery that interleaving improves inductive learning \citep{kornell2008learning}. The importance of dropout for successful imitation has also been noted in animals \citep{galef1988imitation}: ``for the pattern of behaviour initiated by the leader to become part of the behavioural repertoire of the follower, independent of the leader, the pattern of behaviour must come under the control of stimuli not dependent on the presence of the leader''. Humans, along with many animals, have an in-built attentional bias towards biological motion \citep{bardi2011biological, bardi2014first}, mirroring our attention loss (AL). 

Among animals, social learning is known to be preferred over asocial learning in uncertain or varying ecological contexts \citep{aplin2016understanding, smolla2016copy}, environment properties we create via domain randomisation (DR). Learning cultural transmission, then, requires that the environment remains consistently in a ``Goldilocks zone'' of variability, as observed in autocatalytic models \citep{boyd1988culture} and empirical data on climate across human evolution \citep{richerson2005evolution, zachos2001trends}. We achieve this balance by varying the distributional parameters for domain randomisation automatically (A) as a function of the current cultural transmission capability of the agent, keeping the agent in the zone of proximal development \citep{vygotsky1980mind}.

There has been much laboratory work studying cultural transmission in humans, including in situations where humans learn a new behaviour and transmit this behaviour across generations (e.g. \cite{DBLP:journals/corr/abs-2107-13377, saldana2019cumulative, kirby2008cumulative}). Modelling in such settings is typically challenging, particularly when it comes to the intricate sensorimotor structure of behaviour which characterises much human tool use \citep{guerin2013}. On the other hand, there is a long history of interaction between cultural evolution and computational systems. In many such systems, the inheritance step is hard-coded directly (e.g. \citep{gabora1995, rendell2010copy, hart2022artificial, bredeche2022social}), pre-defining the abstraction of the behaviours that can be represented, and potentially limiting the open-endedness of the method. \cite{winfield2022experiments} propose a more ``data-driven'' inheritance system, in which imitation is carried out in third-person by an explicit online learning algorithm. Our work takes this one step further: the ability of cultural transmission is itself learned in a rich sensorimotor environment. Therefore, our methods head towards an even more general and scaleable approach to generating cultural transmission in artificial agents, and perhaps even offers inspiration for modelling; see Section \ref{sec:future_work}.

In RL algorithms, it is common to explore in the space of actions, such as in $\epsilon$-greedy and softmax policies, or when entropy regularisation is used. To overcome local optima in hard exploration problems, authors have proposed exploring in the space of policies via diversity objectives \citep{hong2018diversity}, in the space of states via intrinsic motivation \citep{vamshicuriosity, bellemare2016unifying, burda2018exploration}, in the space of value functions \citep{osband2019deep,badia2020up} and in the space of neural network weights \citep{plappert2018parameter,fortunato2019noisy}. Less common is work on exploration in the space of structured behaviours pertinent to the task at hand, for instance in hierarchical RL \citep{steccanella2020hierarchical}, the kinds of behaviours that humans naturally exchange during cultural transmission. This work helps to fill the gap, solving a hard exploration problem via within-episode cultural transmission, automatically amenable to human interaction. Since this capability is learned, it can be seen as novel form of ``meta-exploration'' \citep{gupta2018meta, liu2021decoupling}. 

We may characterise our setting as a form of meta-learning problem: learning to learn from other agents. The trained network must be capable of online adaptation \citep{Bottou98onlinelearning} with fixed weights, behaving in a way that is rational in hindsight \citep{morrill2020hindsight}. The reinforcement learning (RL) training can be thought of as embedding in the neural network's weights the logic for a state-machine capable of (approximately) Bayes-optimal cultural transmission at test time \citep{mikulik2020meta}. In our trained agent, we indeed found particular memory neurons that encode a subset of the sufficient statistics required for solving the task \citep{DBLP:journals/corr/abs-1905-03030}. Our chosen task has a periodic structure, generating reliable information that an agent can discover and exploit within an episode. Our agent possesses an LSTM memory \citep{hochreiter1997long} and observes its own reward, inspired by the setup in \citet{wang2016learning, duan2016rl}. Apart from these minimal affordances, we do not require any explicit meta-learning algorithms (e.g., \cite{mitchell2021offline}) to train our cultural transmission policy.  

==> Cultural General Intelligence (Final Copy for arXiv)/results.tex <==
\clearpage
\section{Training and evaluation}
\label{sec:results}

Our agent initialisation and procedural world generation algorithm use seeds for their pseudorandom number generators. We first describe in detail results for individual representative seeds, then provide mean and variance statistics across $10$ seeds in Section \ref{sec:ablation-results}. We distinguish between the \textit{training} CT metric, measured on tasks sampled from the training task distribution, and the \textit{evaluation} CT metric, measured on held-out probe tasks defined in Section \ref{sec:probe_tasks}. In both cases, we compute a scalar CT metric from the per-task CT metrics by taking a uniform average. For further results, see Appendix \ref{app:training}.

\subsection{Training without ADR}

In this experiment, we do not control any task parameter using ADR. We study a simple task consisting of a 4-goal game in a $16 \times 16$ world with no obstacles and flat terrain. Figure~\ref{fig:adr-none} shows the training cultural transmission metric and the agent score as training progresses. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/adr/adr_none.png}
    \caption{Training cultural transmission metric and agent score for training without ADR on 4-goal, $16 \times 16$ world with no obstacles and flat terrain. Colours indicate four distinct phases of agent behaviour: (1) (red) startup and exploration, (2) (blue) learning to follow, (3) (yellow) learning to remember, (4) (purple) becoming independent from expert.}
    \label{fig:adr-none}
\end{figure}

The training cultural transmission metric shows four distinct phases over the training run, each corresponding to a distinct social learning behaviour of the agent. In phase 1 (red), the agent starts to familiarise itself with the task, learns representations, locomotion, and explores, without much improvement in score. In phase 2 (blue), with sufficient experience and representations shaped by the attention loss, the agent learns its first social learning skill of following the expert bot to solve the task. The training cultural transmission metric increases to $0.75$, which suggests pure following. 

In phase 3 (yellow), the agent learns the more advanced social learning skill that we call cultural transmission. It remembers the rewarding cycle while the expert bot is present and retrieves that information to continue to solve the task when the bot is absent. This is evident in a training cultural transmission metric approaching $1$ and a continued increase in agent score. 

Lastly, in phase 4 (purple), the agent is able to solve the task independently of the expert bot. The training cultural transmission metric falls back towards $0$ while the score continues to increase. Together, this suggests that the agent is able to achieve high scores with or without the bot. It has learned an ``experimentation'' behaviour, which involves using hypothesis-testing to infer the correct cycle without reference to the bot, followed by exploiting that correct cycle more efficiently than the bot does, resulting in a continuing increase in score. We do not see this experimentation behaviour emerge in the absence of prior social learning abilities: social learning creates the right prior for experimentation to emerge. Example \href{https://sites.google.com/view/dm-cgi\#h.m5zueafwx4p}{videos} corroborate our observations.

\subsection{Training with single-parameter ADR}
\label{sec:adr-single-param}
In this experiment, we use ADR to increase task complexity appropriately to maintain the Goldilocks zone for the learning of cultural transmission, controlling the world size of the training tasks. Figure~\ref{fig:adr-world-size} shows the training curves for the experiment.

\begin{figure}[h]
    \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/adr/adr_on_world_size.png}
         \label{fig:adr:world_size:upper_boundary}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/adr/adr_on_ct.png}
         \label{fig:adr:world_size:ct}
     \end{subfigure}
    \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/adr/adr_on_score.png}
         \label{fig:adr:world_size:score}
     \end{subfigure}
     \caption{Training curves for training with ADR controlling the world size parameter. (left) The upper boundary of the world size randomisation range, the lower boundary is fixed at $16$. (centre) The cultural transmission metric as measured from training environments and held-out probe tasks. (right) The average avatar score over the training run. Note that the decreasing score does not indicate lower performance, since the maximum achievable score decreases with increasing world size.
     }
     \label{fig:adr-world-size}
\end{figure}

The difference between Figures~\ref{fig:adr-none} and~\ref{fig:adr-world-size} is clear. In Figure~\ref{fig:adr-world-size}, the training cultural transmission increases to near $1$ and remains above $0.7$ for the duration of the experiment without dropping towards $0$. This shows the effect of applying ADR to a single parameter. At the start of training, before the world size upper boundary started to increase, all worlds are of size $16 \times 16$. This is the same as in the previous experiment, and we see the same progression in the training cultural transmission metric through phases 1 to 3 as in Figure~\ref{fig:adr-none}. However, as the training cultural transmission metric increases above a threshold ($0.8$ in this experiment), the upper boundary begins to increase in steps of $1$. This continues until the maximum world size of $37 \times 37$ is reached. The progression of novel tasks prevents the collapse of the CT metric towards $0$: our agent no longer enters phase 4.

\subsection{Training with multi-parameter ADR} \label{sec:full-adr}
In this experiment, we train our best cultural transmission agent by using ADR to control the set of task parameters in Table~\ref{tab:adr-parameters}. The parameters include changes to the world that make navigating the terrain more difficult (world size, bumpiness), additional skills to be learned (vertical and horizontal obstacles), and changes to the expert behaviour (bot speed, dropout transition probability). Together, these parameters interact to create tasks that increase in complexity and decrease in expert reliability.

Figure~\ref{fig:adr-full-training} shows the expansion of the randomisation ranges for all parameters for the duration of the experiment. The training cultural transmission metric is maintained between the boundary update thresholds $0.75$ and $0.85$. We see an initial start-up phase of around 100 hours when social learning first emerges in a small, simple set of tasks. Once the training cultural transmission metric exceeds $0.75$, all randomisation ranges began to expand. Different parameters expand at different times, indicating when the agent has mastered different skills such as jumping over horizontal obstacles or navigating bumpy terrain. For intuition about the meaning of the parameter values, see \href{https://sites.google.com/view/dm-cgi\#h.vwuspybn66tu}{example videos} at different times during training.

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/adr/adr_full_training_curve.png}
    \caption{Expansion of parameter randomisation ranges over time, as controlled by ADR. See Figure \ref{fig:adr-full-training-local-ct} for training CT metrics used to decide whether to expand or contract range boundaries. Note a sharp reduction and prolonged instability in world size upper boundary after 200 hours of training. This is likely due to the lack of coordination between parameter boundaries under ADR.}
    \label{fig:adr-full-training}
\end{figure}

Figure~\ref{fig:adr-full-training-eval-ct} shows the evaluation cultural transmission metric over time. Note that all probe tasks are strictly out-of-distribution: during training the world size never expands to $32 \times 32$, and human demonstrations are qualitatively different from an expert bot. Despite these differences, the evaluation CT metric on empty 4-goal tasks reaches a final value of $0.85$, indicating good generalisation and recall. In the 5-goal tasks, the evaluation CT metric is lower. As we show in Section \ref{sec:evaluation}, our agent is still capable of recall and generalisation with 5 goals, but performance drops off in larger worlds. The prominent `dip' in evaluation cultural transmission metrics after 100 training hours is due to ADR starting to expand randomisation ranges at around 100 training hours. This leads to a momentary drop in social learning ability, which is amplified by the difficulty of evaluation tasks. ADR pauses the expansion until the agent recovers at around 150 hours.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/adr/adr_full_training_eval_ct.png}
    \caption{Evaluation cultural transmission metric in three sets of probe tasks.}
    \label{fig:adr-full-training-eval-ct}
\end{figure}

\subsection{Evaluation via ablations}
\label{sec:ablation-results}

Via ablations, we identify a minimal sufficient set of representational and experiential biases which give rise to cultural transmission. The five ingredients are memory (M), expert demonstrations (E), dropout (D), an attention loss (AL), and automatic (A) domain randomisation (DR). We refer to an agent trained with all of these ingredients as MEDAL-ADR. In this section, we ablate each component in turn, showing their impact on performance and cultural transmission capability in empty and complex probe tasks. For more details, see Appendix \ref{app:ablation}. 

For all our ablations, we plot the score achieved throughout training along with the training and evaluation cultural transmission metrics. We report the mean performance for each of these measures across $10$ initialisation seeds for agent parameters and task procedural generation. The shaded area on the graphs represents one standard deviation. We also report the expert's score and the best seed for scale and upper bound comparisons. Figures \ref{fig:ablate-0-agents}, \ref{fig:ablate-dropout} and \ref{fig:ablate-adr} show the results.

\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.27\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ablations/ablate-0-agents-score.png}
        \label{subfig:ablate-0-agents-a}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.27\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ablations/ablate-0-agents-local-ct.png}
        \label{subfig:ablate-0-agents-b}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.27\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ablations/ablate-0-agents-simple-probes.png}
        \label{subfig:ablate-0-agents-c}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ablations/ablate-legend-0-agents.png}
    \end{subfigure}
    \caption{Three different ablated agents, each trained without one crucial ingredient: without an expert (M––––), memory (–EDAL), or attention loss (MED––). The evaluation CT is calculated on empty world $5$-goal probe tasks. All of these agents fail to even partially solve the task (left). They are unable to rely on social cues to acquire cultural information during training (centre) and, consequently, during testing (right). The result for M–––– shows that our task space presents a hard exploration challenge, since this is a pure RL baseline.}
    \label{fig:ablate-0-agents}
\end{figure}

\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.27\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ablations/ablate-dropout-score.png}
        \label{subfig:ablate-dropout-a}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.27\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ablations/ablate-dropout-local-ct.png}
        \label{subfig:ablate-dropout-b}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.27\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ablations/ablate-dropout-simple-probes.png}
        \label{subfig:ablate-dropout-c}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ablations/ablate-legend-dropout.png}
    \end{subfigure}
    \caption{Isolating the importance of expert dropout, we compare our MEDAL agent with the ablated ME–AL agent. ME–AL is more sample efficient (left), but MEDAL achieves higher CT during training (centre) and when evaluated on empty world $5$-goal probe tasks (right). This is because MEDAL is capable of within-episode recall, whereas ME-AL is not. ME-AL represents the previous state-of-the-art method \citep{ndousse2020learning}.}
    \label{fig:ablate-dropout}
\end{figure}

\begin{figure}[H]
    \centering
    \begin{subfigure}[b]{0.27\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ablations/ablate-adr-score.png}
        \label{subfig:ablate-adr-a}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.27\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ablations/ablate-adr-local-ct.png}
        \label{subfig:ablate-adr-b}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.27\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ablations/ablate-adr-complex-probes.png}
        \label{subfig:ablate-adr-c}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.15\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/ablations/ablate-legend-adr.png}
    \end{subfigure}
    \caption{Isolating the automatic (A) and domain randomisation (DR) components, we show that our MEDAL-ADR agent outperforms the ablated MEDAL-–DR and MEDAL-––– agents. The evaluation CT metric is computed in complex world $5$-goal probe tasks (right).  MEDAL-–DR is competitive only on some tasks, while MEDAL-––– hardly learns. Thanks to its adaptive curriculum, MEDAL-ADR achieves the best score and the highest CT.
    }
    \label{fig:ablate-adr}
\end{figure}

==> acknowledgements.tex <==
\section*{Acknowledgements}
\label{acknowledgements}

We would like to thank many, both at DeepMind and in the wider community, for the conversations that have helped to shape this manuscript. We are particularly grateful to (in alphabetical order by last name): Lucy Aplin, Michael Azzam, Jakob Bauer, Satinder Baveja, Charles Blundell, Andrew Bolt, Kalesha Bullard, Max Cant, Nando de Freitas, Seb Flennerhag, Antonio Garcia Castañeda, Thore Graepel, Abhinav Gupta, Nik Hemmings, Max Jaderberg, Natasha Jaques, Andrei Kashin, Simon Kirby, Tom McGrath, Hamza Merzic, Alexandre Moufarek, Kamal Ndousse, Sherjil Ozair, Patrick Pilarski, Drew Purves, Thom Scott-Phillips, Ari Strandburg-Peshkin, DJ Strouse, Kate Tolstaya, Karl Tuyls, Marcus Wainwright, and Jane Wang. 


















==> defns.tex <==
%
% A useful set of commands
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{booktabs}
\usepackage{xfrac}
\usepackage{bbm}

\usepackage{algorithm}
\usepackage{algorithmicx}

\usepackage[most]{tcolorbox}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{changepage}
\usepackage{enumitem}

\newcommand{\qedwhite}{\hfill \ensuremath{\Box}}

%http://www-db.stanford.edu/~manku/latex.html
%The itemize environment can be replaced by:
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }

%Example usage: \squishlist    %% \begin{itemize}
%\item First item
%\item Second item
%\squishend     %% \end{itemize}

\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}


\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}



\newcommand{\tm}{\tilde{m}}
\newcommand{\tv}{\tilde{v}}

% For bold vector symbols
\newcommand{\myvec}[1]{\boldsymbol{#1}}
\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\ind}[1]{\mathbb{I}(#1)}

\newcommand{\vzero}{\myvecsym{0}}
\newcommand{\vone}{\myvecsym{1}}
\newcommand{\valpha}{\myvecsym{\alpha}}
\newcommand{\vbeta}{\myvecsym{\beta}}
\newcommand{\vchi}{\myvecsym{\chi}}
\newcommand{\vdelta}{\myvecsym{\delta}}
\newcommand{\vDelta}{\myvecsym{\Delta}}
\newcommand{\vepsilon}{\myvecsym{\epsilon}}
\newcommand{\vell}{\myvecsym{\ell}}
\newcommand{\veta}{\myvecsym{\eta}}
\newcommand{\vgamma}{\myvecsym{\gamma}}
\newcommand{\vGamma}{\myvecsym{\Gamma}}
\newcommand{\vmu}{\myvecsym{\mu}}
\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vkappa}{\myvecsym{\kappa}}
\newcommand{\vlambda}{\myvecsym{\lambda}}
\newcommand{\vLambda}{\myvecsym{\Lambda}}
\newcommand{\vLambdaBar}{\overline{\vLambda}}
\newcommand{\vomega}{\myvecsym{\omega}}
\newcommand{\vOmega}{\myvecsym{\Omega}}
\newcommand{\vphi}{\myvecsym{\phi}}
\newcommand{\vPhi}{\myvecsym{\Phi}}
\newcommand{\vpi}{\myvecsym{\pi}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\myvecsym{\Psi}}
\newcommand{\vtheta}{\myvecsym{\theta}}
\newcommand{\vTheta}{\myvecsym{\Theta}}
\newcommand{\vsigma}{\myvecsym{\sigma}}
\newcommand{\vSigma}{\myvecsym{\Sigma}}
\newcommand{\vtau}{\myvecsym{\tau}}
\newcommand{\vupsilon}{\myvecsym{\upsilon}}
\newcommand{\vxi}{\myvecsym{\xi}}

\newcommand{\vxn}{\vx^{(n)}}

\newcommand{\vmuY}{\vb}
\newcommand{\vmuMu}{\vmu_{x}}
\newcommand{\vmuMuGivenY}{\vmu_{x|y}}
\newcommand{\vSigmaMu}{\vSigma_{x}}
\newcommand{\vSigmaMuInv}{\vSigma_{x}^{-1}}
\newcommand{\vSigmaMuGivenY}{\vSigma_{x|y}}
\newcommand{\vSigmaMuGivenYinv}{\vSigma_{x|y}^{-1}}
\newcommand{\vSigmaY}{\vSigma_{y}}
\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

%\newcommand{\vmuY}{\vmu_{y}}
%\newcommand{\vmuMu}{\vmu_{\mu}}
%\newcommand{\vmuMuGivenY}{\vmu_{\mu|y}}
%\newcommand{\vSigmaMu}{\vSigma_{\mu}}
%\newcommand{\vSigmaMuInv}{\vSigma_{\mu}^{-1}}
%\newcommand{\vSigmaMuGivenY}{\vSigma_{\mu|y}}
%\newcommand{\vSigmaMuGivenYinv}{\vSigma_{\mu|y}^{-1}}
%\newcommand{\vSigmaY}{\vSigma_{y}}
%\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

\newcommand{\muY}{\mu_{y}}
\newcommand{\muMu}{\mu_{\mu}}
\newcommand{\muMuGivenY}{\mu_{\mu|y}}
\newcommand{\SigmaMu}{\Sigma_{\mu}}
\newcommand{\SigmaMuInv}{\Sigma_{\mu}^{-1}}
\newcommand{\SigmaMuGivenY}{\Sigma_{\mu|y}}
\newcommand{\SigmaMuGivenYinv}{\Sigma_{\mu|y}^{-1}}
\newcommand{\SigmaY}{\Sigma_{y}}
\newcommand{\SigmaYinv}{\Sigma_{y}^{-1}}

\newcommand{\hatf}{\hat{f}}
\newcommand{\haty}{\hat{y}}
\newcommand{\const}{\mbox{const}}
\newcommand{\sigmoid}{\mbox{sigm}}

\newcommand{\one}{(1)}
\newcommand{\two}{(2)}

\newcommand{\va}{\myvec{a}}
\newcommand{\vb}{\myvec{b}}
\newcommand{\vc}{\myvec{c}}
\newcommand{\vd}{\myvec{d}}
\newcommand{\ve}{\myvec{e}}
\newcommand{\vf}{\myvec{f}}
\newcommand{\vg}{\myvec{g}}
\newcommand{\vh}{\myvec{h}}
\newcommand{\vj}{\myvec{j}}
\newcommand{\vk}{\myvec{k}}
\newcommand{\vl}{\myvec{l}}
\newcommand{\vm}{\myvec{m}}
\newcommand{\vn}{\myvec{n}}
\newcommand{\vo}{\myvec{o}}
\newcommand{\vp}{\myvec{p}}
\newcommand{\vq}{\myvec{q}}
\newcommand{\vr}{\myvec{r}}
\newcommand{\vs}{\myvec{s}}
\newcommand{\vt}{\myvec{t}}
\newcommand{\vu}{\myvec{u}}
\newcommand{\vv}{\myvec{v}}
\newcommand{\vw}{\myvec{w}}
\newcommand{\vws}{\vw_s}
\newcommand{\vwh}{\hat{\vw}}
\newcommand{\vx}{\myvec{x}}
%\newcommand{\vx}{\myvec{x}}
\newcommand{\vxt}{\myvec{\tilde{x}}}
\newcommand{\vy}{\myvec{y}}
\newcommand{\vyt}{\myvec{\tilde{y}}}
\newcommand{\vz}{\myvec{z}}

\newcommand{\vA}{\myvec{A}}
\newcommand{\vB}{\myvec{B}}
\newcommand{\vC}{\myvec{C}}
\newcommand{\vD}{\myvec{D}}
\newcommand{\vE}{\myvec{E}}
\newcommand{\vF}{\myvec{F}}
\newcommand{\vG}{\myvec{G}}
\newcommand{\vH}{\myvec{H}}
\newcommand{\vI}{\myvec{I}}
\newcommand{\vJ}{\myvec{J}}
\newcommand{\vK}{\myvec{K}}
\newcommand{\vL}{\myvec{L}}
\newcommand{\vM}{\myvec{M}}
\newcommand{\vN}{\myvec{N}}
\newcommand{\vO}{\myvec{O}}
\newcommand{\vP}{\myvec{P}}
\newcommand{\vQ}{\myvec{Q}}
\newcommand{\vR}{\myvec{R}}
\newcommand{\vS}{\myvec{S}}
\newcommand{\vT}{\myvec{T}}
\newcommand{\vU}{\myvec{U}}
\newcommand{\vV}{\myvec{V}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\vX}{\myvec{X}}
%\newcommand{\vXs}{\vX_{\vs}}
\newcommand{\vXs}{\vX_{s}}
\newcommand{\vXt}{\myvec{\tilde{X}}}
\newcommand{\vY}{\myvec{Y}}
\newcommand{\vZ}{\myvec{Z}}


\newcommand{\vxtest}{\myvec{x}_*}
\newcommand{\vytest}{\myvec{y}_*}


\newcommand{\ftrue}{f_{true}}

\newcommand{\myprec}{\mbox{prec}}
\newcommand{\precw}{\lambda_{w}} % precision of weights (alpha)
\newcommand{\precy}{\lambda_{y}} % precision of y (beta)
\newcommand{\fbar}{\overline{f}}
\newcommand{\xmybar}{\overline{x}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\zbar}{\overline{z}}
\newcommand{\vxbar}{\overline{\vx}}
\newcommand{\vXbar}{\overline{\vX}}
\newcommand{\vybar}{\overline{\vy}}
\newcommand{\vYbar}{\overline{\vY}}
\newcommand{\vzbar}{\overline{\vz}}
\newcommand{\vZbar}{\overline{\vZ}}
\newcommand{\xbar}{\overline{x}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\Ybar}{\overline{Y}}
\newcommand{\Gbar}{\overline{G}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Nbar}{\overline{N}}
%\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\Sbar}{\overline{S}}
\newcommand{\vSbar}{\overline{\vS}}
\newcommand{\Rbar}{\overline{R}}

\newcommand{\vtaubar}{\overline{\vtau}}
\newcommand{\vtbar}{\overline{\vt}}
\newcommand{\vsbar}{\overline{\vs}}

\newcommand{\htilde}{\tilde{h}}
\newcommand{\vhtilde}{\tilde{\vh}}
\newcommand{\Dtilde}{\tilde{D}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\wtilde}{\tilde{w}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\pemp}{p_{emp}}
\newcommand{\pstar}{p^*}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\Xtilde}{\tilde{X}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\vxtilde}{\tilde{\vx}}
\newcommand{\vytilde}{\tilde{\vy}}
\newcommand{\ztilde}{\tilde{\z}}
\newcommand{\vztilde}{\tilde{\vz}}
\newcommand{\vthetaMAP}{\hat{\vtheta}_{MAP}}
\newcommand{\vthetaS}{\vtheta^{(s)}}
\newcommand{\vthetahat}{\hat{\vtheta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\overline{\theta}}
\newcommand{\vthetabar}{\overline{\vtheta}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\vpibar}{\overline{\vpi}}


%\newcommand{\subsubsubsection}[1]{\paragraph{#1}}
\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\real}{\mathbb{R}}

\newcommand{\given}{\|}
\newcommand{\indep}[2]{{#1} \perp {#2}}
\newcommand{\condindep}[3]{{#1} \perp {#2} | {#3}}
\newcommand{\condindepG}[3]{{#1} \perp_G {#2} | {#3}}
\newcommand{\condindepP}[3]{{#1} \perp_p {#2} | {#3}}
\newcommand{\depend}[2]{{#1} \not \perp {#2}}
\newcommand{\conddepend}[3]{{#1} \not \perp {#2} | {#3}}

\newcommand{\trans}[1]{{#1}^{\mathtt{T}}}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
%\newcommand{\rv}{r.v.}
\newcommand{\la}{\leftarrow}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\st}{\mbox{  s.t.  }}

\newcommand{\dom}{\mbox{dom}}
\newcommand{\bel}{\mbox{bel}}
\newcommand{\dsep}{\mbox{dsep}}
\newcommand{\sep}{\mbox{sep}}
\newcommand{\entails}{\models}
\newcommand{\range}{\mbox{range}}
\newcommand{\myspan}{\mbox{span}}
\newcommand{\nullspace}{\mbox{nullspace}}
\newcommand{\adj}{\mbox{adj}}

\newcommand{\nbd}{\mbox{nbd}}
\newcommand{\nbr}{\mbox{nbr}}
\newcommand{\anc}{\mbox{anc}}
\newcommand{\desc}{\mbox{desc}}
\newcommand{\pred}{\mbox{pred}}
\newcommand{\nondesc}{\mbox{nondesc}}
\newcommand{\pa}{\pi}
\newcommand{\ch}{\mbox{ch}}
\newcommand{\mb}{\mbox{mb}}
\newcommand{\connects}{\sim}


\newcommand{\betadist}{\mbox{Beta}}
\newcommand{\Betadist}{\mbox{Beta}}
\newcommand{\bernoulli}{\mbox{Ber}}
\newcommand{\Ber}{\mbox{Ber}}
\newcommand{\Binom}{\mbox{Bin}}
\newcommand{\NegBinom}{\mbox{NegBinom}}
\newcommand{\binomdist}{\mbox{Bin}}
\newcommand{\cauchy}{\mbox{Cauchy}}
\newcommand{\DE}{\mbox{DE}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\discrete}{\calM}
\newcommand{\Discrete}{\calM}
\newcommand{\expdist}{\mbox{Exp}}
\newcommand{\expon}{\mbox{Expon}}
\newcommand{\gammadist}{\mbox{Ga}}
\newcommand{\Ga}{\mbox{Ga}}
\newcommand{\gauss}{{\cal N}}
\newcommand{\IG}{\mbox{IG}}
\newcommand{\IGauss}{\mbox{InvGauss}}
\newcommand{\IW}{\mbox{IW}}
\newcommand{\Laplace}{\mbox{Lap}}
\newcommand{\Mu}{\mbox{Mu}}
\newcommand{\Multi}{\mbox{Mu}}
\newcommand{\NIX}{NI\chi^2}
\newcommand{\GIX}{NI\chi^2}
\newcommand{\NIG}{\mbox{NIG}}
\newcommand{\GIG}{\mbox{NIG}}
\newcommand{\NIW}{\mbox{NIW}}
\newcommand{\GIW}{\mbox{NIW}}
\newcommand{\MVNIW}{\mbox{NIW}}
\newcommand{\NW}{\mbox{NWi}}
\newcommand{\MVNIG}{\mbox{NIG}}
\newcommand{\NGdist}{\mbox{NG}}
\newcommand{\prob}{p}
\newcommand{\Poi}{\mbox{Poi}}
\newcommand{\Student}{{\cal T}}
\newcommand{\student}{{\cal T}}
\newcommand{\Wishart}{\mbox{Wi}}
\newcommand{\Wi}{\mbox{Wi}}
\newcommand{\unif}{\mbox{U}}
\newcommand{\etr}{\mbox{etr}}

\newcommand{\softmax}{\calS}
\newcommand{\soft}{\mbox{soft}}
\newcommand{\cond}{\mbox{cond}}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\matlab}{{\sc MATLAB}}
\newcommand{\NETLAB}{{\sc NETLAB}}
\newcommand{\MLABA}{\mbox{PMTK}}
\newcommand{\BLT}{\mbox{PMTK}}
\newcommand{\PMTK}{\mbox{PMTK}}
\newcommand{\mywp}{\mbox{wp}}

\newcommand{\KLpq}[2]{\mathrm{KL}\left[{#1}\|{#2}\right]}
\newcommand{\KL}{\mbox{KL}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MIxy}[2]{\mathbb{I}\left({#1};{#2}\right)}
\newcommand{\MIxyz}[3]{\mathbb{I}\left({#1};{#2}|{#3}\right)}
\newcommand{\entropy}[1]{\mathbb{H}\left({#1}\right)}
\newcommand{\entropypq}[2]{\mathbb{H}\left({#1}, {#2}\right)}


\newcommand{\vvec}{\mbox{vec}}
\newcommand{\kron}{\otimes}
\newcommand{\dof}{\mbox{dof}}
%\newcommand{\E}{E}
\newcommand{\E}{\mathbb{E}}
\newcommand{\energy}{E}
\newcommand{\expectAngle}[1]{\langle #1 \rangle}
%\newcommand{\expect}[1]{\mathbb{E}\left[ {#1} \right]}
\newcommand{\expect}[2]{\mathds{E}_{{#1}} \left[ {#2} \right]}
\newcommand{\expectGiven}[3]{\mathds{E}_{{#1}} \left[ {#2} \mid {#3} \right]}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\VarGiven}[3]{\mbox{Var}_{{#1}}\left[ {#2} \mid {#3}\right]}
%\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}[1]{\mbox{var}\left[{#1}\right]}
\newcommand{\std}[1]{\mbox{std}\left[{#1}\right]}
\newcommand{\varQ}[2]{\mbox{var}_{{#2}}\left[{#1}\right]}
\newcommand{\cov}[1]{\mbox{cov}\left[{#1}\right]}
%\newcommand{\mode}[1]{\mbox{mode}\left[{#1}\right]}
\newcommand{\median}[1]{\mbox{median}\left[{#1}\right]}



\newcommand{\diag}{\mbox{diag}}
\newcommand{\blkdiag}{\mbox{blkdiag}}
\newcommand{\bias}{\mbox{bias}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}

\newcommand{\size}{\mbox{size}}
\newcommand{\trace}{\mbox{trace}}


\newcommand{\myc}{c}
\newcommand{\myi}{i}
\newcommand{\myj}{j}
\newcommand{\myk}{k}
\newcommand{\myn}{n}
\newcommand{\myq}{q}
\newcommand{\mys}{s}
\newcommand{\myt}{t}


\newcommand{\supp}{\mbox{supp}}


\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calDx}{{\cal D}_x}
\newcommand{\calE}{{\cal E}}
\newcommand{\cale}{{\cal e}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calHX}{{\cal H}_X}
\newcommand{\calHy}{{\cal H}_y}
\newcommand{\calI}{{\cal I}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\caln}{{\cal n}}
\newcommand{\calNP}{{\cal NP}}
\newcommand{\calMp}{\calM^+}
\newcommand{\calMm}{\calM^-}
\newcommand{\calMo}{\calM^o}
\newcommand{\Ctest}{C_*}
\newcommand{\calL}{{\cal L}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calq}{{\cal q}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calSstar}{\calS_*}
\newcommand{\calT}{{\cal T}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calv}{{\cal v}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}

\newcommand{\Lone}{$\ell_1$}
\newcommand{\Ltwo}{$\ell_2$}

\newcommand{\mya}{\mbox{a}}
\newcommand{\myat}{\alpha_{t|t-1}}
\newcommand{\score}{\mbox{score}}
\newcommand{\AIC}{\mbox{AIC}}
\newcommand{\BIC}{\mbox{BIC}}
\newcommand{\BICcost}{\mbox{BIC-cost}}
\newcommand{\scoreBIC}{\mbox{score-BIC}}
\newcommand{\scoreBICL}{\mbox{score-BIC-L1}}
\newcommand{\scoreL}{\mbox{score-L1}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mbox{do}}
\newcommand{\data}{\calD}
\newcommand{\model}{\calM}
\newcommand{\dataTrain}{\calD_{\mbox{train}}}
\newcommand{\dataTest}{\calD_{\mbox{test}}}
\newcommand{\dataValid}{\calD_{\mbox{valid}}}
\newcommand{\futuredata}{\tilde{\calD}}
\newcommand{\algo}{\calA}
\newcommand{\fitAlgo}{\calF}
\newcommand{\predictAlgo}{\calP}
\newcommand{\err}{\mbox{err}}
\newcommand{\logit}{\mbox{logit}}
\newcommand{\parent}{\mbox{pa}}


%%%%%%%%%%% Hoyt

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{n}


\newcommand{\condSet}{\mathcal{S}}
\newcommand{\condSetC}{\mathcal{\lnot S}}


